The G\"ottsche conjecture and the G\"ottsche--Yau--Zaslow formula

The aim of these notes is to give an account, intended for the non-specialist, of the two proofs of the G\"ottsche conjecture given, respectively, first by Tzeng, and shortly after by Kool, Shende and Thomas. Given a smooth, complex, projective surface $S$ and a positive integer $\delta$, the G\"ottsche conjecture predicts that if $L$ is a sufficiently positive line bundle on $S$, then the number of $\delta$-nodal curves in a general $\delta$-dimensional linear subsystem $\Lambda\subset |L|$ is given by a universal polynomial of degree $\delta$ in the four numbers $L^2$, $L K_S$, $K_S^2$, and $c_2(S)$. Besides, the G\"ottsche--Yau--Zaslow formula expresses the generating function of the aforementioned numbers of $\delta$-nodal curves in terms of three explicit quasimodular forms and two unknown universal power series, whose coefficients can be determined by recursion.

==> Bastianelli_Goettsche_Conjecture.tex <==
% \input{enumTV}

% \begin{document}


\chaptitle{The G\"ottsche conjecture
  and the G\"ottsche--Yau--Zaslow formula}
\chapauthor{Francesco Bastianelli and Thomas Dedieu}

\startchap
\label{12.fra-goettsche}

\bandeaupub


% \title[G\"ottsche conjecture and G\"ottsche--Yau--Zaslow formula]
% \author{Francesco Bastianelli}
% \address{Francesco Bastianelli, Dipartimento di Matematica, Universit\`a degli Studi di Bari, Via Edoardo Orabona 4, 
% 70125 Bari, Italy.}
% \email{francesco.bastianelli@uniba.it}

% \author{Thomas Dedieu}
% \address{Thomas Dedieu, Institut de Math\'ematiques de Toulouse -- UMR5219, Universit\'e de Toulouse -- CNRS, UPS IMT, F-31062 Toulouse Cedex 9, France.}
% \email{thomas.dedieu@math.univ-toulouse.fr}



\renewcommand{\HS}[1]{S^{[#1]}}



\let\plbinom\binom
\def\binom#1#2{\textstyle\plbinom{#1}{#2}}

\newenvironment{suspens}{\begingroup\color{gray}}{\endgroup}
\renewenvironment{comment}{\begingroup\color{blue}\itshape}{\endgroup}
\newcommand{\note}[1]{{\color{blue}#1}}
\newcommand{\alarm}[1]{{\color{red}#1}}
\newcommand{\purgatoire}[1]{{\color{gray}#1}}



\begin{abstract}
The aim of these notes is to give an account, intended for the
non-specialist, of the two proofs of the Göttsche conjecture given,
respectively, first by Tzeng, and shortly after by Kool, Shende and
Thomas.

Given a smooth, complex, projective surface $S$ and a positive integer
$\delta$, the G\"ottsche conjecture predicts that if $L$ is a sufficiently
positive line bundle on $S$, then the number of $\delta$-nodal curves
in a general $\delta$-dimensional linear subsystem $\Lambda\subset |L|$ is
given by a universal polynomial of degree $\delta$ in the four numbers
$L^2$, $L K_S$, $K_S^2$, and $c_2(S)$.

Besides, the G\"ottsche--Yau--Zaslow formula expresses the generating
function of the aforementioned numbers of $\delta$-nodal curves in
terms of three explicit quasimodular forms and two unknown universal
power series, whose coefficients can be determined by recursion.
\end{abstract}


\startcontents[12.fra-goettsche]
\renewcommand{\tocdataformat}[1]{\null}
\printcontents[12.fra-goettsche]{}{1}[2]{}



\section{Introduction}


The main theme of this note is the set of enumerative conjectures stated and discussed by G\"ottsche in \cite{G}.
We retrace and summarize the proofs of the G\"ottsche conjecture
given first by Tzeng \cite{T}, and shortly after by
Kool, Shende and Thomas \cite{KST-12}.
We also discuss the proof of the G\"ottsche--Yau--Zaslow formula given
by Tzeng.
Accordingly, \cite{G}, \cite{KST-12} and \cite{T} are the main sources
for this note, and the proofs given here are directly inspired by
those included in the original papers.  

% \medskip
Let $S$ be a smooth complex projective surface, and let $\delta$ be a positive integer.
A $\delta$-\emph{nodal} curve on $S$ is a reduced (possibly reducible)
curve $C\subset S$ having exactly $\delta$ nodes
(\ie ordinary double points), and no other singularities.  
Given a line bundle $L$ on $S$, we denote by $a_{\delta}(S,L)$ the number of $\delta$-nodal curves contained in a general linear subsystem $\Lambda\subset |L|$ of dimension $\delta$.
When $L$ is sufficiently ample, $\delta$-nodal curves in $|L|$ indeed occur in codimension $\delta$, so that $a_{\delta}(S,L)$ is a finite number; moreover, it coincides with the number of $\delta$-nodal curves passing through $\dim |L|-\delta$ general points of $S$,
see \cite[p.234]{KP1-12}, reproduced in
\cite[Lemma \tref{lem:myfav}]{14.th-vainsencher}.
The study of $a_{\delta}(S,L)$ is a very classical theme, and the main topic of this note.
We refer the reader to \cite{KP2-12,KST-12,T},
and \cite{14.th-vainsencher} in this volume,
for a detailed bibliography and a treatise of the background underlying the results we are going to discuss.

% \medskip
The first result we would like to present is the so-called G\"ottsche conjecture \cite[Conjecture 2.1]{G}.
In the light of \cite{Vei,KP1-12}
(described in \cite{14.th-vainsencher})
where formulas for the numbers $a_{\delta}(S,L)$ were given for all
$\delta\leqslant 8$, it predicts that if the line bundle $L$ on $S$ is
sufficiently ample with respect to $\delta$, then the number
$a_{\delta}(S,L)$ is computed by a universal polynomial of degree
$\delta$ in the numbers $L^2, LK_S, K_S^2, c_2(L)$
(universal means that the same polynomial works for all pairs
$(S,L)$).
G\"ottsche's conjecture has been proved in terms of the following positivity notion for a line bundle $L$ on $S$.
\begin{definition}\label{definition VA}
Let $L$ be a line bundle on a smooth projective surface $S$, and let $k\geqslant 0$ be an integer. 
We say that $L$ is $k$-\emph{very ample} if for any $0$-dimensional subscheme $Z\subset S$ of length $k+1$, the restriction map $H^0(S,L)\to H^0(Z, L\otimes \mathcal{O}_Z)$ is surjective.
\end{definition}

\noindent
The G\"ottsche conjecture was first proved by Tzeng \cite{T}.
Shortly after, Kool, Shende and Thomas proved the following version
(see \cite[Theorem 4.1]{KST-12}),
with weaker positivity assumptions on $L$.

\begin{theorem}[G\"ottsche conjecture]\label{theorem KST}
For all positive integers $\delta$, there exists a polynomial $T_{\delta}(x,y,z,t)$ of degree $\delta$ with the following property: for any smooth complex projective surface $S$ and for any $\delta$-very ample line bundle $L$ on $S$, a general $\delta$-dimensional linear subsystem $\Lambda\subset |L|$ contains exactly $T_{\delta}(L^2,LK_S,K_S^2,c_2(S))$ $\delta$-nodal curves, \ie
\begin{equation}\label{eq KST}
a_{\delta}(S,L)=T_{\delta}(L^2,LK_S,K_S^2,c_2(S)).
\end{equation}
\end{theorem}

It is worth noting that the coefficients of the polynomial
$T_{\delta}(x,y,z,t)$ may be computed for all $\delta$.
% $\geqslant 0$
% (we set $T_{0}(x,y,z,t)=1$, which is the number $a_0(S,L)$ when $L$ is sufficiently positive). 
Indeed, the numbers $a_{\delta}(S,L)$ can be determined for all line bundles on $\P^2$ by \cite[Theorem 1.1]{CH-12}, and for all primitive line bundles on a $K3$ surface by \cite[Theorem 1.1]{BL-12};
moreover, the 4-tuple of topological invariants $(L^2, LK_S, K_S^2, c_2(L))$ is $(n^2,-3n,9,3)$ if $(S,L)=\left(\P^2,\mathcal{O}_{\P^2}(n)\right)$, and $(L^2,0,0,24)$ if $L$ is a primitive line bundle on a $K3$ surface $S$;
it follows that the coefficients of each $T_{\delta}(x,y,z,t)$ can be computed by solving a system of linear equations obtained from \eqref{eq KST} using different values of $n$ and $L^2$.  


\medskip
We will discuss the two proofs of Theorem \ref{theorem KST} given
by Tzeng \cite{T}, and Kool, Shende, and Thomas \cite{KST-12},
respectively.
There is also another proof due to Liu \cite{Liu1,Liu2}, but we will
not report on it.
The Kool--Shende--Thomas proof is close in spirit to the work of
Vainsencher and Kleiman--Piene on node polynomials, which is 
described in \cite{14.th-vainsencher}.
In particular it enables one to compute explicitly the node
polynomials $T_\delta$ although, in its authors' own words, it is
not terribly efficient.
Tzeng's proof, on the other hand, involves an abstract version of the
degeneration methods constituting the backbone of this volume,
see, in particular, \cite{01.ciro} and \cite{04.concettina}.

We retrace the Kool--Shende--Thomas proof
in Section \ref{section KST}. It relies on
BPS calculus on Hilbert schemes of points on
(arbitrary reduced) curves on a surface $S$,
see \cite{PT,S}, the calculation of tautological integrals on Hilbert schemes of points on $S$ by means of the recursion introduced in \cite{EGL},
and the deformation theory of plane singularities of curves,
see, \eg \cite{DH} and \cite{02.edoardo}.
The main idea underlying the proof is to describe the numbers
$a_{\delta}(S,L)$ of $\delta$-nodal curves in a general linear
subsystem $\Lambda\subset |L|$ in terms of the Euler characteristics
of relative Hilbert schemes of points associated to the universal
curve $\mathcal{C}\to \Lambda$.
This is what BPS calculus is used for;
after that, the proof consists in (non-trivial) intersection theoretic considerations.
We refer to the introduction of Section \ref{section KST}
for a more detailed outline.

We survey Tzeng's proof
in Section \ref{section T}.
Ultimately, it relies on the fact, proved in
\cite{levine-morel},
that the algebraic cobordism group of smooth, complex, projective
surfaces is generated by (the classes of)
$\P^2$ and $\P^1\times\P^1$.
Tzeng's proof is formulated in the framework of
\cite{LevP,LeeP} for algebraic cobordism, which is based on the notion
of (extended) double point relation: roughly speaking, one mods out the
free abelian group generated by all smooth surfaces by relations
corresponding to degenerations of one surface to the transverse union
of two surfaces.
Tzeng's main result is a suitable version of Jun Li's celebrated
degeneration formula in this context,
which involves Li and Wu's construction of
a moduli space of stable ideal sheaves in \cite{LW}.
The degeneration formula enables her to express the numbers $a_\delta$
for the pair $(S,L)$
(actually, the better suited variant $d_\delta(S,L)$ introduced by
Göttsche) in terms of the numbers $a_\delta$ for the generators of the
algebraic cobordism group, which then leads to the Göttsche conjecture.


\medskip
The other results we will discuss concern the
structure of the generating function of
the universal polynomials $T_{\delta}(L^2,LK_S,K_S^2,c_2(S))$, that is
the
following formal power series in $x$,
\begin{equation*}
T(S,L):=\sum_{\delta\geqslant 0} T_{\delta}(L^2,LK_S,K_S^2,c_2(S))\, x^{\delta}
\end{equation*}
(we set $T_{0}(x,y,z,t)=1$).
In \cite{G} G\"ottsche proved that if the numbers $a_{\delta}(S,L)$ are indeed computed by universal polynomials, then the function $T(S,L)$ must satisfy rather strong conditions. 
In particular, it has the following
multiplicative structure by \cite[Proposition 2.3]{G},
which we may now state unconditionally since
the G\"ottsche conjecture is proved.

\begin{theorem}\label{theorem G}
There exist universal power series $A_1,A_2,A_3,A_4\in \Q[[x]] ^\times$ such that
\begin{equation*}
T(S,L)=A_1^{L^2}A_2^{LK_S}A_3^{K_S^2}A_4^{c_2(S)}.
\end{equation*}
\end{theorem}

\noindent
We emphasize that the power series $A_i$ are invertible in $\Q[[x]]$
(in fact, their constant coefficients all equal $1$), so their
exponentiations 
are defined unambiguously.

G\"ottsche's proof of this fact consists in considering a pair $(S,L)$ obtained as the disjoint union of pairs of the form $(\P^2, \mathcal{O}_{\P^2}(n))$ and $(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1}(n,n))$, and using the additivity properties of the 4-tuples $(L^2,LK_S,K_S^2,c_2(S))$.
We will give Tzeng's proof in Section \ref{sub proofs};
it formulates the same idea in the
somehow taylor-made theory of algebraic cobordism.

We further point out that, as was the case for the coefficients of the
universal polynomials $T_{\delta}(x,y,z,t)$, the coefficients of the
universal power series $A_1,A_2,A_3,A_4$ may be determined by the
recursive formulas describing the numbers $a_{\delta}(S,L)$ for
certain classes of pairs $(S,L)$ (see, \eg the aforementioned
\cite[Theorem 1.1]{CH-12} for line bundles on $\P^2$ and \cite[Theorem
6.7]{Vak} for the case of Hirzebruch surfaces).


\medskip
Another important result concerning the generating function $T(S,L)$ is the G\"ottsche--Yau--Zaslow formula, which was conjectured by G\"ottsche \cite{G} based on the formulas in \cite{Vei,KP1-12}, as a generalization of the Yau--Zaslow formula for rational curves on $K3$ surfaces \cite{YZ-12}, see \cite{10.th-panoramico}.
In particular, the G\"ottsche--Yau--Zaslow formula expresses the
universal power series $T(S,L)$ in terms of five universal generating
functions in one variable $q$: three explicit quasimodular forms, and
two unknown universal power series, whose coefficients may
nevertheless be determined by the recursion formula of \cite{CH-12}.   

We refer the reader to \cite{KZ} for some preliminary notions on modular and quasimodular forms.
Let $\tau\in \mathbb{C}$ be a complex number with positive imaginary part, and set $q:=e^{2\pi i\tau}$. 
Consider the \emph{discriminant form} 
$$
\Delta(\tau):= q\prod_{n>0}\left(1-q^n\right)^{24}
$$
and the \emph{second Eisenstein series} 
$$
G_2(\tau):=-\frac{1}{24}+\sum_{n>0}\bigg(\sum_{k|n}k\bigg)q^n,
$$
which are a modular form and a quasimodular form, respectively. 
Furthermore, given the differential operator $D:=\frac{1}{2\pi i}\frac{d}{d\tau}=q\frac{d}{dq}$, we have that for any quasimodular form $f$, the derivative $Df$ is again a quasimodular form. 
Then the following holds, see \cite[Conjecture 2.4]{G} and
\cite[Theorem 1.2]{T}.

\begin{theorem}[G\"ottsche-Yau--Zaslow formula]\label{theorem T}
There exist universal power series $B_1(q)$ and $B_2(q)$ such that 
\begin{equation*}
  \sum_{\delta\geqslant 0}  T_{\delta}(L^2,LK_S,K_S^2,c_2(S))
  \cdot
  DG_2(\tau)^{\delta}
=\frac{\left(DG_2(\tau)/q\right)^{\chi(L)}B_1(q)^{K_S^2}B_2(q)^{LK_S}}{\left(\Delta(\tau)D^2G_2(\tau)/q^2\right)^{\chi(\mathcal{O}_S)/2}}.
\end{equation*}
\end{theorem}

We give the proof in Section \ref{sub proofs}.
An essential input in it is Bryan and Leung's main result in
\cite{BL-12}, see \cite{10.th-panoramico}.


We note that, according to \cite[Remark 2.6]{G} and \cite[Corollary 4.4]{T}, the G\"ottsche--Yau--Zaslow formula can be reformulated as follows. 
For a smooth projective surface $S$ and for any $l,m,r\in \Z$, we define 
$$N_r^S(l,m):=T_{l+\chi(\mathcal{O}_S)-1-r}(2l+m,m,K_S^2,c_2(S)).$$ 
Then Theorem \ref{theorem T} gives that
$$\sum_{l\in \Z}N_r^S(l,m)q^l=B_1(q)^{K_S^2}B_2(q)^m(DG_2(\tau))^r\frac{D^2G_2(\tau)}{\left(\Delta(\tau)D^2G_2(\tau)/q^2\right)^{\chi(\mathcal{O}_S)/2}},$$ 
and Theorem \ref{theorem KST} ensures that if $L$ is a $\delta$-very ample line bundle on $S$ with $\delta=\chi(L)-1-r$, then the coefficient $N_r^S\left(\frac{L^2-LK_S}{2},LK_S\right)$ counts the number of $\delta$-nodal curves in a general linear subsystem $W\subset |L|$ of codimension $r$. 
Analogously, setting $g=\frac{L^2+LK_S}{2}+1-\delta$, the coefficient
$$
\begin{array}{c}
M_g^S\left(\frac{L^2-LK_S}{2},LK_S\right):=N_{g-m-2+\chi(\mathcal{O}_S)}\left(\frac{L^2-LK_S}{2},LK_S\right)
\end{array}
$$
computes the number of nodal curves of geometric genus $g$ in a general linear subsystem of $|L|$ having codimension $r=g-LK_S-2+\chi(\mathcal{O}_S)$.

\medskip
To conlude this introduction, let us mention some further
developments, which we will not discuss any more in the text.
Using the BPS calculs described in
Section \ref{sub euler characteristic},
Göttsche and Shende \cite{goettsche-shende-12},
see also \cite{goettsche-shende2-12},
defined refined counting invariants, which interpolate between the
usual counts over the complex numbers and Welschinger invariants;
this, in turn, influenced tropical counts by Block-Goettsche
\cite{block-goettsche-A-12}.

Kleiman and Piene have further conjectured that 
Theorem \ref{theorem KST} should hold more generally for a relative
family of curves in a family of surfaces: this has been proved by
Laarakker \cite{laarakker},
by elaborating on the proof of Kool--Shende--Thomas.
Rennemo \cite{rennemo-12} has furthermore proved a generalization of
Theorem \ref{theorem KST}
valid for all isolated singularity types and in all dimensions, again
following the way opened by Kool--Shende--Thomas.


\paragraph*{Acknowledgements}
The first author would like to thank Giulio Codogni, Lothar
G\"ottsche, Manfred Lehn, Donatella Iacono, Margarida Melo, and
Filippo Viviani, for helpful discussions and explanations during the
preparation of a series of lectures on this topic and during the
writing of this note.

The second author thanks Laurent Manivel
and Adrien Sauvaget for their help with the
Ellingsrud--G\"ottsche--Lehn recursion,
and the first author for everything.

We both thank Martijn Kool and Richard Thomas for their comments on
this text.


\begin{notation}
We work throughout over the field $\C$ of complex numbers. 
By \emph{curve} we mean a connected complete reduced algebraic curve, unless otherwise stated.
% When we speak of a \emph{smooth} projective variety, we implicitly assume it to be irreducible.

Given a projective variety $X$, we say that a property holds for a \emph{general} point ${x\in X}$ if it holds on an open non-empty subset of $X$.
In particular, if $L$ is a line bundle on a smooth surface $S$, by \emph{general} linear subsystem $\Lambda\subset |L|$ of dimension $\delta$ we mean that $\Lambda$ is parameterized over an open subset of the Grassmannian of $\delta$-dimensional linear subspaces of $|L|\simeq \P^{h^0(L)-1}$.

For a positive integer $k$, we denote by $X^{[k]}$ the $k$-fold Hilbert scheme of points on a variety $X$, parameterizing $0$-dimensional subschemes of $S$ of length $k$, and by $\Hilb^k(\mathcal{X}/B)$ the $k$-fold relative Hilbert scheme of points on the fibres of a family $\mathcal{X}\to B$ of varieties. 

The \emph{Euler number} (sometimes Euler characteristic)
of a topological space $X$ is the number
$e(X) = \sum _i (-1)^i \dim H_c^i(X,\Z)$,
where the subscript $c$ means cohomology with compact support.
We refer to \cite[Section \tref{s:pencil}]{10.th-panoramico} for some
basic properties of the Euler number, including its additivity,
and an expression when $X$ is a fibration.
\end{notation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Kool--Shende--Thomas' proof of the G\"ottsche conjecture}
\label{section KST}

%Introduzione con spiegazione dei passaggi salienti della dimostrazione e del fatto che la sezione 2 seguirò Shende
In this section, we present the proof of Theorem \ref{theorem KST} given by Kool, Shende, and Thomas \cite{KST-12}.
So, we consider a line bundle $L$ on a smooth surface $S$, and we assume that $L$ is $\delta$-very ample for some integer $\delta\geqslant 1$.
%Let $a_\delta(S,L)$ be the number of $\delta$-nodal curves (counted with multiplicity) contained in a general linear subsystem of $V\subset |L|$ of dimension $\delta$.

In \S \ref{sub ample linear systems}, we show that a general,
$\delta$-dimensional, linear subsystem $\Lambda$ of $|L|$ contains a
finite number of $\delta$-nodal curves, each occurring with
multiplicity 1, and that all the other elements of $\Lambda$ are
reduced curves having larger geometric genus.
This is an application of the deformation theory of plane curve
singularities, using in an essential way the
$\delta$-very ampleness of $L$.

In \S \ref{sub euler characteristic}, we first review some facts
concerning the generating functions  of the Euler characteristics
$e(C^{[k]})$ of Hilbert schemes of points on curves $C$,
for any reduced curve $C$ contained in $S$;
this is the so-called BPS calculus on Hilbert schemes of points.
We then use these facts to express the number $a_\delta(S,L)$ of $\delta$-nodal curves in
a general $\Lambda\subset |L|$ as a linear combination of the Euler
numbers $e(\Hilb^k(\mathcal{C}/\Lambda))$,
$k=0,\dots,\delta$,
of the relative Hilbert schemes of points on the fibres of the universal curve $\mathcal{C}\to \Lambda$.
This is done by stratifying $\Lambda$ according to the topological
types of its members, and using the additivity of the Euler number.

In \S \ref{sub tautological}, we conclude the proof by showing that
each term appearing in this linear combination is indeed a polynomial in $L^2$, $LK_S$, $K_S^2$ and $c_2(L)$. 
To this aim, we retrace Kool--Shende--Thomas' computation of the Euler
numbers $e(\Hilb^k(\mathcal{C}/\Lambda))$ in terms of certain
tautological integrals,
first on the Hilbert schemes $S^{[k]}$,
and then on the products $S^k$.

The passing from integrals on  $S^{[k]}$ to integrals on $S^k$
relies on the recursion of Ellingsrud, G\"ottsche and Lehn
\cite[Sections 3 and 4]{EGL}, which we survey in
\S \ref{s:EGL}.

\paragraph{}
\label{p:KST-idea}
We point out that the idea underlying this count of $\delta$-nodal curves generalizes the following argument for the case $\delta=1$
(it is explained in more details in
\cite[Section \tref{s:pencil}]{10.th-panoramico}).
Assume that $L$ is a very ample line bundle and $\Lambda\subset |L|$ is a general pencil, and denote by $p$ the genus of the smooth fibres of the universal curve $\mathcal{C}\to \Lambda\cong \P^1$. 

The quantity $e(C)-(2-2p)$ equals 1 if $C$ is 1-nodal, 
and 0 if $C$ is smooth.
Therefore, summing this quantity over $\Lambda\cong \P^1$, we obtain
the identity
\begin{equation*}
  % \label{eq a_1}
a_1(S,L)=e(\mathcal{C})-(2-2p)\,e(\P^1).
\end{equation*}
To see this formula as a particular case of the
Kool--Shende--Thomas' count, we 
rewrite it in terms of linear combinations of Euler
characteristics of Hilbert schemes of points:
one has
\begin{equation*}
  e(C)-(2-2p)
  = e(C^{[1]})-(2-2p)\,e_0(C^{[0]})
\end{equation*}
and, correspondingly,
\begin{equation*}
  e(\mathcal{C})-(2-2p)\,e(\P^1)
  = e(\Hilb^1(\mathcal{C}/\Lambda)) -
  (2-2p)\, e(\Hilb^0(\mathcal{C}/\Lambda)).
\end{equation*}

In \S \ref{sub euler characteristic},
we give a similar expression of
$a_\delta(S,L)$ as a sum over
all members $C$ of $\Lambda\cong \P^\delta$ of
some linear combination of
the Euler characteristics $e(C^{[k]})$,
$k=1,\dots,\delta$, which
takes value $1$ for $\delta$-nodal curves, and $0$ for curves having
higher geometric genus.  
So, in order to prove the G\"ottsche conjecture, it remains to express
the corresponding linear combination of the Euler numbers
$e(\Hilb^k(\mathcal{C}/\Lambda))$, $k=0,\ldots,\delta$,
% (for $\delta=1$, this is the right-hand-side of \eqref{eq a_1})
in
terms of the topological invariants $L^2$, $L K_S$, $K_S^2$ and
$c_2(S)$; this is the purpose of \S \ref{sub tautological}.

For $\delta=1$, this goes simply as follows:
$e(\mathcal{C})=c_2(S)+L^2$ as $\mathcal{C}$ is the blow-up of $S$ at $L^2$ points, $2p-2=L(L+K_S)$ by the adjunction formula, and $e(\P^1)=2$, so that we obtain 
$$a_1(S,L)=c_2(S)+3L^2+2L K_S,$$   
which is indeed a polynomial of degree 1 in the topological numbers $L^2,L K_S, K_S^2,c_2(S)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Sufficiently ample line bundles}
\label{sub ample linear systems}

Let $L$ be a line bundle on a smooth projective surface $S$.
We follow \cite[Section 2]{KST-12} to show how the $\delta$-very
ampleness condition on $L$
ensures that the singularities
of curves in a general dimension $\delta$ linear subsystem $\Lambda\subset
|L|$
behave sufficiently well
for the count of $\delta$-nodal curves in $\Lambda$ by
means of the Euler numbers $e(\Hilb^k(\mathcal{C}/\Lambda))$ in
subsection~\ref{sub euler characteristic}
to make sense, see Theorem \ref{theorem KST3.4}.
Roughly speaking, the singularities of the members of
$\Lambda$ behave as expected up to codimension $\delta$ in $|L|$.
The precise statement is the following.
%Following \cite[Section 2]{KST-12}, we prove  \cite[Proposition
%2.1]{KST-12} (see Theorem \ref{theorem KST2.1} below) concerning
%singular curves contained in a general linear subsystem $V\subset
%|L|$, provided that $L$ is a sufficiently positive line bundle on a
%smooth surface $S$.


\begin{theorem}
\label{theorem KST2.1}
Assume $L$ is $\delta$-very ample for some positive integer
$\delta$. 
Let $p$ denote the common arithmetic genus of all members of $|L|$,
and consider a general linear subsystem $\Lambda \subset |L|$ of
dimension $\delta$. 
Then all members of $\Lambda$ are reduced curves, and have geometric
genus $g \geq p-\delta$.
Moreover, there are finitely many members of genus
$g=p-\delta$; they are all $\delta$-nodal curves,
and appear with multiplicity $1$.
\end{theorem}


Let us clarify the last sentence.
Recall that the locus $V^\delta(\Lambda)$ parametrizing $\delta$-nodal
members of $\Lambda$ is well-defined as a subscheme of $\Lambda$,
see \cite{DS-12} for a discussion and the relevant references;
the locus $V_{g}(\Lambda)$ parametrizing genus $g$ members of
$\Lambda$, however, is only defined set-theoretically (it is a
{locally closed subset} of $\Lambda$).
Now, the last sentence means that
(i) the set $V_{p-\delta}(\Lambda)$ has dimension $0$
and coincides with the support of
$V^\delta(\Lambda)$,
and (ii) the scheme $V^\delta(\Lambda)$ is reduced.


\begin{remark}
\label{rk:thm-KST2.1}
Note that the theorem implies that all members of $\Lambda$ have at
most $\delta$ singular points, and all members with $\delta$ singular
points are $\delta$-nodal curves. Indeed, each singular point makes
the geometric genus drop by at least one.
\end{remark}

% Let $L$ be a line bundle on a smooth projective surface $S$ and let $p$ be 
% If $L$ is $\delta$--very ample for some integer $\delta> 0$, then the

%  contains a finite number of $\delta$--nodal curves, each appearing with multiplicity 1.
% Moreover, all the other curves in $V$ are reduced with geometric genus $g>p-\delta$.  

% \begingroup
% % redéfinition boîteuse de paragraph
% \renewcommand{\theparagraph}{\thesubsection.\arabic{paragraph}}
% \def\step{\refstepcounter{paragraph}
% \medskip\noindent
% \theparagraph.\ }

% \begin{proof}
The rest of Section \ref{sub ample linear systems} is dedicated to the
proof of Theorem \ref{theorem KST2.1}.
We will use extensively the deformation theory of planar curve singularities,
for which we refer to \cite{02.edoardo} in this volume, and to \cite{DH,GLS-12}
for extended treatises; the reader may also consult \cite{DS-12}.
The punchline is that the $\delta$-very ampleness property ensures
that the maps from the relevant equigeneric and equisingular subloci
of  $|L|$ to the corresponding semi-universal deformation spaces
of singularities are smooth,
because their differentials are restriction maps,
and the $\delta$-very ampleness grants their surjectivity.


% \step
\paragraph{}
\label{pr:delta-nodal}
Let us first show that the subscheme $V^\delta(|L|) \subset |L|$ of
$\delta$-nodal curves in $|L|$ is smooth of codimension $\delta$. 
By Bertini's theorem this implies that
$V^\delta(\Lambda) = V^\delta(|L|) \cap \Lambda$ is smooth of
dimension $0$, \ie
$\delta$-nodal curves in
$\Lambda$ are finitely many and appear with multiplicity $1$.

Let $[C] \in |L|$ be a $\delta$-nodal curve, and 
$J$ be its Jacobian ideal.
The vector space $B:=H^0\left(C, \mathcal{O}_C/J\right)$ is the
product of the semi-universal deformation spaces of the various
singularities of $C$.
We thus have a map of pointed germs $\varphi: (|L|,[C]) \to (B,0)$,
and its differential is the restriction map
\begin{equation*}
%\label{diff:versal-map}
\rho_J:
T_{|L|, [C]} \cong H^0(S,L)/ \langle s_C \rangle 
\longrightarrow
H^0\left(Z, L\otimes \O_C/J \right),
\end{equation*}
where $Z \subset S$ is the singular subscheme of $C$, defined in $C$
by the ideal $J$, 
and $s_C \in H^0(S,L)$ is a section with zero divisor equal to $C$.
Since $C$ is $\delta$-nodal, its singular subscheme has length
$\delta$, hence the restriction map
$H^0(S,L) \to H^0(Z,L \otimes \O_Z)$ is surjective by the
positivity property of $L$.
This implies that the map
% \eqref{diff:versal-map}
$\rho_J$
is surjective, hence
$\varphi$ is smooth.

The semi-universal deformation space of a node is a line, in which the
equisingular locus is only the origin.
Thus the locus of $\delta$-nodal curves in $B$ is only the origin,
which is smooth and has codimension $\delta$ in $B$.
By smoothness of $\varphi$, the same holds for $V^\delta(|L|)$ around
$[C]$, which proves our claim.

% Let us set $\P:=\P\left(H^0(S,L)\right)\cong |L|$, and
% let $[s]\in \P$ be a point parameterizing a $\delta$--nodal
% curve $C\subset S$ in $|L|$.
% Given a polynomial $f\in \C[x,y]$ providing a local equation
% of $C$ at its singular points, we may consider a miniversal
% deformation space $B:=H^0\left(C, \mathcal{O}_C/J\right)$ of the
% singularities of $C$, where $J:=\left(\frac{\partial f}{\partial x},
% \frac{\partial f}{\partial y}\right)$ is the Jacobian ideal of $f$. 

% Hence the germ of the space $\P$ at $[s]$ admits a map $(\P,[s])\stackrel{\varphi}{\longrightarrow} (B,0)$ to the deformation space. % passare al fascio di ideali e definire J.
% Being $T_{[s]}\P\cong H^0(S,L)/\langle s\rangle$, % (see \eg \cite[Example 16.1]{Harris})
% the tangent map induced by $\varphi$ is $H^0(S,L)/\langle s\rangle\stackrel{T_\varphi}{\longrightarrow} H^0\left(Z, L\otimes \mathcal{O}_Z\right)$, where $Z\subset S$ is the 0--dimensional scheme of length $\delta$ defined by $\mathcal{O}_C/J$ and supported at the singularities of $C$.
% In particular, the tangent map fits in the diagram
% \begin{equation*}
% \xymatrix{H^0(S,L) \ar[d] \ar[dr]^{\gamma_Z} & \\ H^0(S,L)/\langle s\rangle \ar[r]^-{T_\varphi} & H^0\left(Z, L\otimes \mathcal{O}_Z\right),}
% \end{equation*}
% where $\gamma_Z$ is the restriction map appearing in Definition \ref{definition VA}, which is surjective as the line bundle $L$ is $(\delta-1)$--very ample by assumption.
% Thus $T_\varphi$ is surjective, which implies that $\varphi$ is a
% smooth morphism.

% Since $C$ is a $\delta$--nodal curve, the equisingular locus is the
% locus of $\delta$--nodal curves in $B$, and it coincides with the
% equigeneric locus, which is smooth and has codimension $\delta$ in
% $B$. 
% % We recall that the deformation space $B$ contains the
% % \emph{equigeneric locus} $\mathrm{EG}\subset B$, which is supported on
% % the points of $B$ parameterizing deformations of $C$ having the same
% % geometric genus as $C$, and the \emph{equisingular locus}
% % $\mathrm{ES}\subset \mathrm{EG}$, which---roughly
% % speaking---parameterizes deformations having the same topological type
% % as $C$.
% Therefore, the smoothness of $\varphi$ ensures that the locus of
% $\delta$--nodal curves in $\P$ is smooth of codimension
% $\delta$.  It follows that its intersection with a general
% $\delta$--dimensional linear subspace of $\P$ consists of
% finitely many reduced points, \ie a general linear subsystem
% $V\subset |L|$ of dimension $\delta$ contains a finite number of
% $\delta$--nodal curves, each appearing with multiplicity 1.

% \step
\paragraph{}
\label{step:cog>delta}
Consider a non-negative integer $g'<p-\delta$, and let 
$V_{g'}(|L|) \subset |L|$ be the locally closed subset of reduced curves having
geometric genus $g'$.
We now show that $V_{g'}(|L|)$ has codimension
(strictly) greater than $\delta$ in $|L|$, which implies that
$\Lambda$ does not contain any curve of genus $g'$. 

Let $[C] \in V_{g'}(|L|)$. We consider its conductor ideal $A$, and let $Y$ be the subscheme of $C$ defined by $A$.
By \cite[Proposition 3.1]{02.edoardo} the tangent cone of $V_{g'}(|L|)$ at $[C]$
is contained in the kernel of the restriction map
\[
\rho_Y: H^0(S,L)/ \langle s_C \rangle
\longrightarrow
H^0 \left(Y, L\otimes \mathcal{O}_{C}/A \right),
\]
where $s_C$ is again a section with zero divisor equal to $C$.

Since the co-genus $p-g'$ of $C$ in $|L|$ is greater than $\delta$, we may find a
subscheme $Z \subset Y$ of length $\delta+1$.
Then the positivity property of $L$ implies that the restriction map
\[
\rho_Z: H^0(S,L)/ \langle s_C \rangle
\longrightarrow
H^0 \left(Z, L\otimes \mathcal{O}_{Z} \right)
\]
is surjective, hence its kernel has codimension $\delta+1$. Since 
$\rho_Z = \pi \circ \rho_Y$, where $\pi$ is the restriction map 
$H^0(L\otimes \O_Y) \to H^0 (L\otimes \O_Z)$, this implies that the
kernel of $\rho_Y$ has codimension at least $\delta+1$, hence $V_{g'}(|L|)$ has
codimension at least $\delta +1$ in $|L|$ as required.

% \smallskip
% (ii) Now, we focus on the locus in $\P$ parameterizing reduced
% curves having geometric genus $g<p-\delta$.  So, let $s\in H^0(S,L)$
% be a section defining such a curve $C\in |L|$.  Let $A$ denote the
% conductor ideal (see \cite{02.edoardo}), and let $Y\subset S$ be the
% $0$-dimensional scheme of length $p-g>\delta$ defined by
% $\mathcal{O}_{C}/A$.  According to \cite[Proposition 3.1]{02.edoardo}, the
% locus in $\P$ described by (possibly locally trivial)
% deformations of $C$ with geometric genus $g$ has tangent cone
% contained in the kernel of the map $H^0(S,L)/\langle
% s\rangle\stackrel{\psi}{\longrightarrow} H^0\left(Y, L\otimes
% \mathcal{O}_{Y}\right)$.  By arguing as above, we consider a subscheme
% $Z\subset Y$ of length $\delta +1$ and the composition
% $H^0(S,L)/\langle s\rangle\stackrel{\phi_Z}{\longrightarrow}
% H^0\left(Z, L \otimes \mathcal{O}_Z\right)$ of $\psi$ with the natural
% restriction map.  Thus $\phi_Z$ is surjective as $L$ is a
% $\delta$-very ample line bundle, and we deduce that $\codim \ker
% \psi\geqslant\delta +1$.  Therefore, we conclude that the locus in
% $\P$ parameterizing reduced curves having geometric genus
% $g<p-\delta$ has codimension at least $\delta +1$, as wanted.

% \step
\paragraph{}
\label{pr:worse-sings}
Let $\tau$ be a collection of topological types of planar
singularities, which does not consist of
$\delta$ nodes, and such that a member of $|L|$ with singularities of
type $\tau$ has genus $p-\delta$. 
We now show that the subscheme $V^\tau(|L|) \subset |L|$ parametrizing
curves with topological type $\tau$ has codimension (strictly) greater than  $\delta$ in $|L|$.

Let $[C] \in V^\tau(|L|)$, and $I$ be its equisingular ideal.
By \cite[Proposition 3.1]{02.edoardo}, the tangent space to $V^\tau(|L|)$ at $[C]$
is the kernel of the restriction map
\[
\rho_Y: H^0(S,L)/ \langle s_C \rangle
\longrightarrow
H^0 \left(Y, L\otimes \mathcal{O}_{C}/I \right),
\]
where $Y$ is the subscheme of $C$ defined by $I$.
The assumptions on $\tau$ imply that we may find a subscheme $Z
\subset Y$ of length $\delta+1$, see \cite[Lemma~2.4]{02.edoardo}.
Then, as in \ref{step:cog>delta},
the $\delta$-very ampleness of $L$ implies that the kernel of $\rho_Y$
has codimension
at least $\delta+1$, hence $V^\tau(|L|)$ has codimension
at least $\delta+1$ in
$|L|$ as claimed.

\providecommand{\nr}{\mathrm{nr}}
% \step
\paragraph{}
\label{p:tg-to-discr}
Finally, we proceed to show that the locus $V^\nr(|L|) \subset |L|$
parametrizing non-reduced curves has codimension
(strictly) greater than $\delta$.

We claim that if $C$ is a non-reduced member of $|L|$, then the
tangent cone to $V^\nr(|L|)$ at $[C]$ is contained in the 
kernel of the restriction map
\[
\rho: H^0(S,L)/ \langle s_C \rangle
%\stackrel{\psi}
\longrightarrow
H^0\left(C_\mathrm{red}, L\otimes
\mathcal{O}_{C_\mathrm{red}}\right).
\]
When we know this, we conclude that $V^\nr(|L|)$ has codimension
greater than $\delta$
always along the same lines: we pick a
$0$-dimensional subscheme $Z \subset C_\red$ of length $\delta+1$, 
and the kernel of $\rho$ is contained in the kernel of the
restriction to $Z$, which has codimension $\delta+1$ since $L$ is
$\delta$-very ample.

To prove our claim, we argue as in \cite[\S 2.1]{V2} and consider the
incidence variety 
\[
\cD:=
\left\{
\bigl( [C],p \bigr) \in |L|\times S:
C\ 
\text{is singular at}\ 
p
\right\}.
\]
It is smooth: indeed since $L$ is very ample and $S$ is smooth, $\cD$
is a projective bundle over $S$.
On the other hand, if $[C] \in V^\nr(|L|)$ then 
$([C],p) \in \cD$ for all $p \in C_\red$.
It follows that the tangent cone to $V^\nr(|L|)$ at $[C]$ is contained in
the image of the tangent space to $\cD$ at $([C],p)$ by
the projection $T_{|L|\times S} \to T_{|L|}$ for all $p \in C_\red$.
We shall show that the latter image is contained in the kernel of the
restriction 
\[
H^0(S,L)/ \langle s_C \rangle
%\stackrel{\psi}
\longrightarrow
H^0\bigl(p, \restr L p\bigr),
\]
and this will prove our claim.

The equations of $\cD$ in $|L| \times S$ are as follows. 
Let $([C],p) \in |L|\times S$;
we choose a local system of coordinates $(x,y)$ on $S$ around $p$, 
and see $|L|$ around $[C]$ as a finite dimensional affine space of
polynomials $f \in \C[x,y]$.
% in $(x,y)$, around a defining equation  of
% $C \subset S$.
In this representation, $\cD$ is defined 
%around $([C],p)$ 
by the equations
\[
f(x,y)=df(x,y)=0.
% f(0)
% =\partial _x f(0)
% = \partial_y f(0)
% =0.
\]
By differentiation, the latter equations give the equations of the
tangent space of $\cD$ in $T_{|L|}\times T_S$.
In particular, if
$(h,v) \in T_{|L|,f} \times T_{S,(x,y)}$ sits in $T_{\cD}$,
%,(f_C,p)}$,
%where the polynomial $f_C$ respresents $[C]\in |L|$, 
then
\[
df(x,y)(v)+h(x,y)=0,
\]
which is equivalent to $h(x,y)=0$ since $df(x,y)=0$.
In other words, if $([C],p) \in \cD$, then the projection of 
$T_{\cD,([C],p)}$ to $T_{|L|,[C]}$ is contained in the kernel of the
restriction map 
\[
H^0(S,L)/ \langle s_C \rangle
%\stackrel{\psi}
\longrightarrow
H^0\bigl(p, \restr L p\bigr),
\]
as we wanted to prove.
We have thus proved our claim, hence that $V^\nr(|L|)$ has codimension
greater than $\delta$.

%\end{proof}
\bigskip%\noindent
The results proved in
\ref{pr:delta-nodal},
\ref{step:cog>delta},
\ref{pr:worse-sings},
and \ref{p:tg-to-discr}
together amount to Theorem \ref{theorem KST2.1}.
The proof of the latter is therefore complete.
\qed

% \endgroup
% % fin redéfinition boîteuse

% \bigskip
% (i) We firstly consider the case of non-reduced curves. 
% So, let $C\in |L|$ be a non-reduced curve defined by a section $s\in H^0(S,L)$. 
% We claim that the tangent cone at $[s]$ to the sublocus
% $\Sigma\subset\P$ parameterizing non-reduced curves is
% contained in the kernel of the map $T_{[s]}\P\cong
% H^0(S,L)/\langle s\rangle\stackrel{\psi}{\longrightarrow}
% H^0\left(C_\mathrm{red}, L\otimes
% \mathcal{O}_{C_\mathrm{red}}\right)$.
% To see this fact, we argue as in \cite[\S 2.1]{V2} and we consider the
% incidence variety 
% $$
% \mathcal{I}:=\left\{\left([f],Z\right)\in \P\times S^{[\delta]}\left|
% \begin{array}{l}
% Z \text{ is supported at } \delta \text{ distinct points }
% z_1,\dots,z_\delta\in S \\ \text{and }\{f=0\} \text{ is singular at
% }z_i \text{ for all }i=1,\dots,\delta 
% \end{array}\right.\right\}.
% $$
% Let $[f]=(f_0:\ldots:f_r)$ be coordinates on $\P$ with respect
% to a basis $\{s_0,s_1\dots,s_r\}\subset H^0(S,L)$ and let $z=(x,y)$ be
% local coordinates on $S$.
% Setting $F([f],z):=\sum_{i=1}^{r}f_is_i(x,y)\in
% \C[f_0,\ldots,f_r,x,y]$, we have that $\mathcal{I}$ has local
% equations $F([f],z_i)=\frac{\partial F}{\partial
% x}([f],z_i)=\frac{\partial F}{\partial y}([f],z_i)=0$ for all
% $i=1,\dots,\delta$.
% By differentiation, we obtain the equations of the tangent space $T_{([f],Z)}\mathcal{I}\subset T_{[f]}\P\times T_{Z}S^{[\delta]}$.
% In particular, we deduce from the equations $F([f],z_i)=0$ that if
% $(g,v_1+\dots+v_\delta)\in T_{([f],Z)}$, then
% $\left\langle\left(\frac{\partial F}{\partial
% x}([f],z_i),\frac{\partial F}{\partial x}([f],z_i)\right),
% v_i\right\rangle+g(z_i)=0$, and hence $g(z_i)=0$ for all
% $i=1,\dots,\delta$.
% Therefore, denoting by $\pi\colon \mathcal{I}\longrightarrow
% \P$ the natural projection, the tangent cone to
% $\pi(\mathcal{I})$ at a point $[f]$ is contained in the locus
% $$
% \left\{\left.g\in T_{[f]}\P\right|g(z)=0\text{ for any point }z\in S \text{ where } \{f=0\}\text{ is singular}\right\}.
% $$
% Since $C=\{s=0\}$ is a non-reduced curve, $C$ is singular at each of its points. 
% Hence the tangent cone to $\Sigma$ at $[s]$ is contained in the locus of tangent vectors $g\in T_{[s]}\P$ vanishing along $C_\mathrm{red}$, as claimed.

% Given any $0$-dimensional scheme $Z\subset C_\mathrm{red}$ of length $\delta+1$, let $H^0(S,L)/\langle s\rangle\stackrel{\phi_Z}{\longrightarrow} H^0\left(Z, L \otimes \mathcal{O}_Z\right)$ be the composition of $\psi$ with the natural restriction map. 
% Since $L$ is $\delta$-very ample, the map $\phi_Z$ is surjective, so that $\codim \ker \psi\geqslant\codim \ker \phi_Z=\dim \Img \phi_Z=\delta +1$.
% Thus the locus in $\P$ parameterizing non-reduced curves has codimension at least $\delta +1$, as well.

% \smallskip
% (iii) Finally, let us consider the locus in $\P$ corresponding to reduced curves having geometric genus $p-\delta$ and admitting a singularity which is not a node. 
% Let $\Sigma_m\subset \P$ denote the locus parameterizing curves $C\in |L|$ of geometric genus $g=p-\delta$ such that the \emph{total Milnor number} (\ie the sum over the singularities of $C$ of the corresponding Milnor numbers) is $m$.
% We recall that $m\geqslant p-g=\delta$, with $m=\delta$ if and only if $C$ is a $\delta$-nodal curve.
% Therefore $\Sigma_\delta\subset \P$ is the locus parameterizing $\delta$-nodal curves, whereas reduced curves with geometric genus $p-\delta$ and a non-nodal singularity are parameterized by $\bigcup_{m>\delta}\Sigma_m$.

% Fix $m>\delta$, and let $[s]\in \Sigma_m$ be a point corresponding the a curve $C\in |L|$.
% We want to prove that $C$ admits an equigeneric deformation which is not equisingular. 
% By arguing as above, the tangent cone to the locus in $\P$ parameterizing deformations of $C$ with geometric genus $p-\delta$ is contained in the kernel of the map $T_{[s]}\P\cong H^0(S,L)/\langle s\rangle\stackrel{\psi}{\longrightarrow} H^0\left(Y, L\otimes \mathcal{O}_{Y}\right)$, where $A$ is the conductor ideal and $Y\subset S$ is the $0$-dimensional scheme of length $p-g=\delta$ defined by $\mathcal{O}_{C}/A$.
% Since $L$ is $(\delta-1)$-very ample, the map $\psi$ is surjective, and hence the germ of $\P$ at $[s]$ maps transversally to the equigeneric locus in the miniversal deformation space $B:=H^0\left(C, \mathcal{O}_C/J\right)$ \textbf{\emph{(perché mi serve?)}}. 
% Let $I\subset A$ denote the equisingular ideal, which is strictly included in the conductor ideal as $C$ has non-nodal singularities (\cf \cite[Lemma 2.4]{02.edoardo}).
% Then, given a singular point $p\in C$, there exists a non-costant map $A/I\longrightarrow \mathcal{O}_p$, whose kernel defines an ideal $I\subset K\subsetneq A$ with $\mathrm{length}(A/K)=1$.
% Being $\mathrm{length}(\mathcal{O}_{C}/A)=\delta$, we deduce that $\mathcal{O}_{C}/K$ defines a $0$-dimensional scheme $Z\subset S$ of length $\delta+1$,  %(\cf Atiyah Macdonald Proposizione 6.9 p.119) 
% so that the map $H^0(S,L)/\langle s\rangle{\longrightarrow} H^0\left(Z, L\otimes \mathcal{O}_{Z}\right)$ is surjective as $L$ is $\delta$-very ample.\\

% \textbf{\emph{(Inserire parte mancante)}}\\

% Then $C$ admits a family of deformations which is equigeneric but not equisingular.
% Therefore, the general member of such a family is a curve having geometric genus $g=p-\delta$, but total Milnor number smaller than $m$.
% It follows that $[s]\in \Sigma_m$--and hence the whole $\Sigma_m$--lies in the closure of $\Sigma_\delta\cup \Sigma_{\delta+1}\cup\dots\cup\Sigma_{m-1}$.
% Since we proved above that the locus $\Sigma_\delta$ of $\delta$-nodal curves is smooth of codimension $\delta$, we deduce that $\codim\Sigma_m\geqslant \delta+1$ for any $m>\delta$.
% Thus the locus $\bigcup_{m>\delta}\Sigma_m$ of curves with geometric genus $p-\delta$ and a non-nodal singularity has codimension at least $\delta +1$, and this fact concludes the proof.
%  \end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Euler characteristics of Hilbert schemes of points over
  curves}
\label{sub euler characteristic}

We consider a smooth projective surface $S$ endowed with a $\delta$-very ample line bundle $L$ on $S$,
as in Theorem \ref{theorem KST2.1}.
We follow \cite[Section 3]{KST-12} in order to express the number $a_\delta(S,L)$ of $\delta$-nodal curves in a general $\delta$-dimensional linear subsystem $\Lambda\subset |L|$ in terms of Euler numbers $e(\Hilb^k(\mathcal{C}/\Lambda))$ of relative Hilbert schemes, where $\mathcal{C}\to \Lambda$ is the universal curve.

To this aim, we recall a couple of preliminary results describing the
generating series of the Euler characteristics $e(C^{[k]})$ of
$k$-fold Hilbert schemes of points on curves $C\subset S$,
see \cite[Propositions 3.1 and 3.2]{KST-12}.
Both results were first proved in \cite{PT} in the setting of stable pairs, whereas \cite[Section 2]{S} includes proofs using only Hilbert schemes.   
\begin{proposition}\label{proposition KST3.1}
Let $S$ be a smooth surface and let $C\subset S$ be a curve having
arithmetic genus $p$ and geometric genus $g$.
There exists a unique sequence of integers
$(n_{C,g},n_{C,g+1},\dots, n_{C,p})$,
depending only on the topological type of $C$,
such that the generating series of the Euler characteristics
$e(C^{[k]})$ satisfies 
$$
\sum_{k=0}^{\infty} e(C^{[k]})q^k=\sum_{i=g}^{p} n_{C,i} q^{p-i}(1-q)^{2i-2}.
$$
\end{proposition}

Writing the
generating series $\sum e(C^{[k]})q^k$ as a sum $\sum n_{C,i}
q^{p-i}(1-q)^{2i-2}$ with $i$ ranging between $-\infty$ and $p$
is granted by a formal property of power series, see
\cite[Proposition 1]{S}.
However,
the geometry of $C$ is involved in the proof that
$n_{C,i}=0$ for all $i<g$; this is deduced from \cite[Proposition
8]{S}, see \cite[Corollary 11]{S}.

When the curve $C$ is $\delta$-nodal, the generating series of Euler
characteristics $e(C^{[k]})$ is governed by the following,
see \cite[Corollary 12]{S}.
\begin{proposition}\label{proposition KST3.2}
Let $C$ be a $\delta$-nodal curve with arithmetic genus $p$.
Then the coefficients $n_{C,i}$ appearing in Proposition
\ref{proposition KST3.1} are 
$$
n_{C,i}={\binom \delta {p-i}}
$$
for all $i=p-\delta, \ldots, p$. 
\end{proposition}

When $C$ is a smooth curve this was proved by Macdonald
\cite{Macdonald}, in order to give a new proof of the de Jonqui\`eres
formulas discussed in \cite{13.th-classic}. In this case one finds 
\begin{equation*}
%\label{1courbe-lisse}
\sum _{k=0} ^\infty e\bigl( C^{[k]} \bigr) q^k
= (1-q)^{2p-2}
= \sum _{k=0} ^{2p-2} (-1)^k 
{\textstyle
\binom {2p-2} k}
q^k.
\end{equation*}
While $e(C)=2-2p$, and 
$e(C^{[k]})=0$ if $k > 2p-2$ because then $C^{[k]}\to J^k(C)$ gives a
structure of projective bundle over a torus, the values of $e(C^{[k]})$
for $1<k \leq 2p-2$ are not obvious to us.

In the general case of Proposition~\ref{proposition KST3.2}, 
Kool, Shende, and Thomas interpret the number $\binom \delta {p-i}$ as
the number of partial normalizations of $C$ at $p-i$ of its $\delta$
nodes. This is the reason why Proposition~\ref{proposition KST3.2} is
considered a statement in BPS calculus, see \cite{10.th-panoramico}.


\bigskip
We may now state the main result of this section,
see \cite[Theorem 3.4]{KST-12}.
It follows from Propositions
\ref{proposition KST3.1}, \ref{proposition KST3.2} and Theorem
\ref{theorem KST2.1}

\begin{theorem}\label{theorem KST3.4}
Let $S$ be a smooth projective surface equipped with a line
bundle $L$, and denote by
$p$ be the arithmetic genus of all members of $|L|$.  
Let $\delta$ be a positive integer such that $L$ is
$\delta$-very ample, and consider a general linear subsystem $\Lambda\subset
|L|$ of dimension $\delta$.
Let $\mathcal{C}\to \Lambda$ be the universal curve over $\Lambda$.
There are integers
$n_{\Lambda,p-\delta},\ldots,n_{\Lambda,\delta}$ such that the
following identity of formal power series holds:
\begin{equation}\label{eq KST3.4}
\sum_{k=0}^{\infty} e(\Hilb^k(\mathcal{C}/\Lambda))q^k = \sum_{i=p-\delta}^p
n_{\Lambda,i} q^{p-i}(1-q)^{2i-2}.
\end{equation}
Moreover,
the number
$a_\delta(S,L)$ of $\delta$-nodal curves in $\Lambda$ equals  $n_{\Lambda,p-\delta}$.
\end{theorem}

% In applying the second part of this statement, one should
% recall that 
% $p=1+ \frac 1 2 (K_SL+L^2)$
% by the adjunction formula.

\begin{proof}
Let $T$ be the (finite) set indexing the topological types of the
members of $\Lambda$.  For all $\tau\in T$, let
% $V_{\tau}\subset \Lambda$
$V^\tau_\red = V^\tau(\Lambda)_\red$
be
the locus of curves having
topological type $\tau$, and let $g_{\tau}$ denote the common
geometric genus of these curves. 
Note that $g_{\tau}\geqslant p-\delta$ by Theorem \ref{theorem KST2.1}.
Let $\mathcal{C}_\tau\to V^{\tau}_\red$ be the universal curve.

For all $k \geq 0$, the relative Hilbert scheme
$\Hilb^k(\mathcal{C}_\tau/{V^\tau_\red})$ is a topological fibre bundle, so
$\displaystyle e(\Hilb^k(\mathcal{C}_\tau/{V^\tau_\red}))=
e(C_\tau^{[k]})e({V^\tau_\red})$ for any membre $C_\tau$ of $\Lambda$
of topological type $\tau$. 
For all $i=g_\tau,\ldots,p$, we denote by $n_{\tau,i}$ the number
$n_{C_\tau,i}$ as in Proposition \ref{proposition KST3.1}
(it depends only on $\tau$);
we set $n_{\tau,i}=0$ if $i<g_\tau$.
Then, by the additivity of the Euler number, and using Proposition
\ref{proposition KST3.1}, we have
\begin{align*}
\sum_{k=0}^{\infty} e(\Hilb^k(\mathcal{C}/\Lambda))q^k 
& = \sum_{k=0}^{\infty} \Bigl( \sum_{\tau\in T}
  e(C_\tau^{[k]})e(V^\tau_\red)\Bigr) q^k 
= \sum_{\tau\in T}\Bigl(\sum_{k=0}^{\infty} e(C_\tau^{[k]})q^k\Bigr)
e(V^\tau_\red)
= \\
& = \sum_{\tau\in T}\Bigl( \sum_{i=g_\tau}^{p}
n_{\tau,i} q^{p-i}(1-q)^{2i-2}
\Bigr) e(V^\tau_\red)
 = \sum_{i=p-\delta}^{p} n_{\Lambda,i}q^{p-i}(1-q)^{2i-2},
\end{align*}
with $n_{\Lambda,i}:= \sum_{\tau\in T} n_{\tau,i}e(V^\tau_\red)$:
this proves the identity \eqref{eq KST3.4}.

Theorem \ref{theorem KST2.1} ensures that $\delta$-nodal curves are
the only curves in $\Lambda$ having geometric genus $p-\delta$, they are
finitely many, and they appear with multiplicity 1. Therefore
$n_{\Lambda,p-\delta}= a_\delta (S,L)\cdot
n_{\delta A_1,p-\delta}$,
where $\delta A_1$ denotes the topological type of $\delta$-nodal curves members of $|L|$.
Since $n_{\delta A_1,p-\delta}=1$ by Proposition
\ref{proposition KST3.2}, one has
$n_{\Lambda,p-\delta}= a_\delta (S,L)$ as we wanted.
\end{proof}

\begin{corollary}
\label{c:theorem KST3.4}
The number
$a_\delta(S,L)$
is a linear combination of the numbers
$e(\Hilb^k(\mathcal{C}/\Lambda))$, $k=0,\ldots, \delta$, in
which 
the coefficient of $e(\Hilb^k(\mathcal{C}/\Lambda))$ is a polynomial in $p$ of
degree at most $\delta-k$ for all $k$, and the coefficient of
$e(\Hilb^\delta(\mathcal{C}/\Lambda))$ is $1$.
\end{corollary}

\begin{proof}
Let $e_{\Lambda,k} = e(\Hilb^k(\mathcal{C}/\Lambda))$
for all $k=0,\ldots, \delta$.
Expanding $(1-q)^{2i-2}$ for all $i$ in
\eqref{eq KST3.4} gives
\begin{equation*}
  \sum_{k=0}^{\infty} % e(\Hilb^k(\mathcal{C}/\Lambda))
  e_{\Lambda,k}
  q^k = \sum_{i=p-\delta}^p
n_{\Lambda,i} \sum_{m=0}^{2i-2}
{\textstyle \binom {2i-2} m}(-1)^m q^{p-i+m}. 
\end{equation*}
Then, by comparing the coefficients of $q^k$ for $k=0,\dots,\delta$, 
one sees with standard algebraic manipulations that 
\begin{equation}
\label{eq:ek_nv}
% e(\Hilb^k(\mathcal{C}/\Lambda))=
e_{\Lambda,k} =
\sum_{m=0}^k (-1)^m 
{\textstyle \binom {2(p-k+m)-2} m}
n_{\Lambda,p-k+m}. 
\end{equation}


Let us now show by induction on $k=0,\ldots,\delta$ that
\[
n_{\Lambda,p-k} = P_{k,0}(p)\,e_{\Lambda,0} + \cdots + P_{k,k-1}(p) \,
e_{\Lambda,k-1}
+ e_{\Lambda,k},
\]
where each $P_{k,s}$ is a polynomial of degree
at most $k-s$, independent
of $\Lambda$.
The case $k=\delta$ gives the wanted result,
since $a_\delta(S,L) = n_{\Lambda,p-\delta}$
by Theorem \ref{theorem KST3.4}.

For $k=0$ one has
$n_{\Lambda,p} = e_{\Lambda,0}$ by \eqref{eq:ek_nv}, as required.
Suppose now that $k$ is positive.
For all $m=1,\ldots,k$, we set
$Q_{k,m}(p)=(-1)^m {\textstyle \binom {2(p-k+m)-2} m}$,
a polynomial of degree $m$ in $p$.
By \eqref{eq:ek_nv} and our recursion hypothesis, we have 
\begin{equation*}
e_{\Lambda,k}
=  n_{\Lambda,p-k}
+  \sum _{m=1} ^k Q_{k,m}(p) \, 
\sum _{s=0} ^{k-m}  P_{k-m,s}(p) e_{\Lambda,s} 
=  n_{\Lambda,p-k}
+ \sum _{s=0} ^{k-1}
\sum _{m=1} ^{k-s} Q_{k,m}(p) \, 
  P_{k-m,s}(p) e_{\Lambda,s} 
\end{equation*}
(setting $P_{m,m}=1$). This gives an explicit expression for 
$P_{k,s}$, which ends the proof since
\[
\deg (Q_{k,m} P_{k-m,s}) \leq
m + (k-m-s) = k-s.
\]
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Proof of the G\"ottsche conjecture}
\label{sub tautological}
In this section we prove Theorem \ref{theorem KST}, following
\cite[Section 4]{KST-12}.
With Corollary~\ref{c:theorem KST3.4} at hand,
the remaining task is to compute the Euler characteristics
$e(\Hilb^k(\mathcal{C}/\Lambda))$, expressing them as polynomials of
degree $k$ in the numbers $L^2,LK_S,K_S^2,c_2(L)$;
this is done with the recursion of \cite{EGL}.

\begin{proof}[Proof of Theorem \ref{theorem KST}]
Consider a smooth projective surface $S$ and a $\delta$-very ample
line bundle $L$ on $S$.  Let $p$ be the arithmetic genus of the curves
in $|L|$, and let $\Lambda\subset |L|$ be a general linear subsystem of
dimension $\delta$ with universal curve $\mathcal{C}\to
\Lambda$.  Corollary~\ref{c:theorem KST3.4} ensures that the number
$a_\delta(S,L)$ of $\delta$-nodal curves in $\Lambda$ is a linear
combination of the Euler numbers $e(\Hilb^k(\mathcal{C}/\Lambda))$,
$k=0,\ldots, \delta$, where the coefficient of each
$e(\Hilb^k(\mathcal{C}/\Lambda))$ is a polynomial of degree at most
$\delta-k$ in $p$, and the coefficient of
$e(\Hilb^\delta(\mathcal{C}/\Lambda))$ equals 1.  Moreover, these
polynomials are independent of the pair $(S,L)$ and, since
$p=\frac{1}{2}L^2 +\frac{1}{2}K_SL+1$ by the adjunction formula, the
coefficient of $e(\Hilb^k(\mathcal{C}/\Lambda))$ is a polynomial of degree
at most $\delta-k$ in $L^2$ and $K_SL$.  
The G\"ottsche conjecture therefore follows from
Proposition~\ref{P:e(Hilb^k)} below.
\end{proof}

\begin{proposition}
\label{P:e(Hilb^k)}
The Euler characteristics 
$e(\Hilb^k(\mathcal{C}/\Lambda))$ is a polynomial of degree exactly $k$ in
the numbers $L^2,LK_S,K_S^2,c_2(L)$.
% and the degree of
% $e(\Hilb^\delta(\mathcal{C}/\Lambda))$ is exactly $\delta$.
\end{proposition}

\begin{proof}
The case $k=0$ follows from the following equalities:
\[
  e(\Hilb^0(\mathcal{C}/\Lambda))=e(\Lambda)= e(\P^\delta) =\delta+1.
\]
Let us now assume that $1\leqslant k\leqslant \delta$.
We divide the proof in three steps.

\setcounter{step}{0}
\def\step{\refstepcounter{step}%
  \medskip\noindent
  {\itshape Step \thestep.}}

\step{}
We consider the Hilbert scheme $S^{[k]}$ and the universal subscheme $Z_{k}\subset S\times S^{[k]}$, endowed with the projections $\pi_1\colon Z_k\to S$ and $\pi_2\colon Z_k\to S^{[k]}$.
We define a vector bundle $L^{[k]}$ of rank $k$ on $S^{[k]}$,
$$L^{[k]}:={\pi_2}_*\pi_1^*L.$$
Letting $\P:=\P\left(H^0(S,L)\right) = |L|$, we consider the line bundle $L\boxtimes\mathcal{O}_\P(1):=\pi_S^*L\otimes \pi_\P^*\mathcal{O}_\P(1)$ on $S\times \P$, where $\pi_S$ and $\pi_\P$ are the two projections.
In view of the standard identification $H^0(S,L)\otimes H^0(S,L)^*\cong \mathrm{Hom}\left(H^0(S,L),H^0(S,L)\right)$, we may consider the canonical section $\mathrm{id}_{H^0(S,L)}\in H^0(S,L)\otimes H^0(S,L)^*$ of the line bundle $L\boxtimes\mathcal{O}_\P(1)$.
By taking the pullback of $\mathrm{id}_{H^0(S,L)}$ to $S\times S^{[k]}\times \P$, and pushing down to $S^{[k]}\times \P$ its restriction to $Z_k\times \P\subset S\times S^{[k]}\times \P$, we obtain a tautological section of the vector bundle
$M^{[k]}$ on $S^{[k]}\times \P$ defined as
$$M^{[k]}
= L^{[k]} \boxtimes \O_\P(1)
:=\pi_{S^{[k]}}^*L^{[k]}\otimes \pi_\P^*\mathcal{O}_\P(1).$$  

By abuse of notation, we denote by $\mathcal{C}\to \P$ the universal
curve over the complete linear system $|L|$. The relative Hilbert
scheme $\Hilb^k(\mathcal{C}/\P)$ is a smooth subvariety of
$S^{[k]}\times \P$,
of dimension $k+\dim(\P)$ hence codimension $k$ in 
$S^{[k]}\times \P$.
Since it coincides moreover with the vanishing locus of the tautological section
of $M^{[k]}$
corresponding to  $\mathrm{id}_{H^0(S,L)}$,
its class in the Chow ring of $S^{[k]}\times \P$
is
Poincar\'e dual to the Chern class $c_k(M^{[k]})$, that is
$\bigl[\Hilb^k(\mathcal{C}/\P)\bigr]=c_k(M^{[k]})\cap \bigl[S^{[k]}\times \P\bigr]$  (see, \eg \cite[Example 3.2.16]{F}).
We note furthermore that the fibre of the projection $\Hilb^k(\mathcal{C}/\P)\to S^{[k]}$ over any $0$-dimensional scheme $Z\in S^{[k]}$ is given by pairs $(Z,[s])\in S^{[k]}\times \P$ such that $s$ vanishes at $Z$, \ie $s\in \ker \bigl(H^0(S,L)\stackrel{\gamma_Z}{\longrightarrow} H^0\left(Z, L\otimes \mathcal{O}_{Z}\right)\bigr)$. 
As $L$ is $(k-1)$-very ample for all $k=1,\ldots,\delta+1$,
the map $\gamma_Z$ is surjective, so that the tautologial section of $M^{[k]}$ vanishes transversally with respect to the fibration $\Hilb^k(\mathcal{C}/\P)\to S^{[k]}$, whose fibres
therefore have constant dimension.  
Moreover, since the linear subsystem $\Lambda\subset \P$ is general,
% it correspond to a $\delta$-dimensional linear subspace of $H\subset \P$ cut out by general hyperplanes. 
the restriction $\Hilb^k(\mathcal{C}/\Lambda)\subset S^{[k]}\times \Lambda$ is smooth by Bertini's Theorem.
Therefore, since the class $\bigl[\Hilb^k(\mathcal{C}/\Lambda)\bigr]$ is Poincar\'e dual in the Chow ring of $S^{[k]}\times \Lambda$ to the $k$-th Chern class of the restriction of $M^{[k]}$,
the Euler characteristic of $\Hilb^k(\mathcal{C}/\Lambda)$ satisfies
\begin{align*}
  e(\Hilb^k(\mathcal{C}/\Lambda))
  & = \int_{\Hilb^k(\mathcal{C}/\Lambda)} c_k (T_{\Hilb^k(\mathcal{C}/\Lambda)})
 = \int_{\Hilb^k(\mathcal{C}/\Lambda)} c_\bullet
    (T_{\Hilb^k(\mathcal{C}/\Lambda)})
  \\
  &  = \int_{\Hilb^k(\mathcal{C}/\Lambda)}
    \frac{c_\bullet(T_{S^{[k]}\times \Lambda})}
    {c_\bullet(M^{[k]})}
    = \int_{S^{[k]}\times \Lambda} c_k(M^{[k]})
    \frac {c_\bullet(T_{S^{[k]}\times \Lambda})}
    {c_\bullet(M^{[k]})}.
\end{align*}

\step{}
Let us now spell out the various terms in the last integral
above.
Let $\omega=c_1(O_{\Lambda}(1))$ be the hyperplane class on $\Lambda\simeq \P^\delta$. 
One has $c_\bullet(T_\Lambda)=\sum_{k=0}^\delta{\delta+1\choose
  k}\omega^k=(1+\omega)^{\delta+1}$ (see, \eg \cite[p.414]{GH}),
hence
$c_\bullet(T_{S^{[k]}\times \Lambda})
= c_\bullet(T_{S^{[k]}}) c_\bullet(T_{\Lambda})
= c_\bullet(T_{S^{[k]}}) (1+\omega)^{\delta+1}$.

On the other hand, since $M^{[k]}$ is the tensor product of the rank
$k$ vector bundle $\pi_{S^{[k]}}^*L^{[k]}$ with the line bundle
$\pi_\P^*\mathcal{O}_\P(1)$, its restriction to $\Lambda$ satisfies
$c_k(M^{[k]})=\sum_{i=0}^k\omega^ic_{k-i}(L^{[k]})$
(see, \eg \cite[p. 55]{F}).
Finally,  \cite[Example 3.2.2]{F} yields
\begin{align*}
   c_\bullet(M^{[k]})
   & =\sum_{p=0}^k c_p(M^{[k]})=\sum_{p=0}^k
     \biggl(\sum_{i=0}^p {\binom {k-i}{p-i}} c_i(L^{[k]})\omega^{p-i} \biggr)=\\
   &   =\sum_{i=0}^k c_i(L^{[k]})\sum_{p=i}^k  {\binom {k-i}{p-i}}
     \omega^{p-i}=\sum_{j=0}^k c_{k-j}(L^{[k]})(1+\omega)^{j}.
\end{align*}
Thus,
\begin{align}
\label{e(Hilb^k-0}
e(\Hilb^k(\mathcal{C}/\Lambda))
&=\int_{S^{[k]}\times \Lambda}
\frac
{c_\bullet(T_{S^{[k]}}) (1+\omega)^{\delta+1}
\sum_{i=0}^k\omega^ic_{k-i}(L^{[k]})}
{\sum_{j=0}^k
c_{k-j}(L^{[k]})(1+\omega)^{j}}
\\
\label{e(Hilb^k}
&= \int_{S^{[k]}}
\operatorname{Coeff}_{\omega^\delta}
\Bigl( \frac
{c_\bullet(T_{S^{[k]}}) (1+\omega)^{\delta+1}
\sum_{i=0}^k\omega^ic_{k-i}(L^{[k]})}
{\sum_{j=0}^k
c_{k-j}(L^{[k]})(1+\omega)^{j}}
\Bigr).
\end{align}
% so that $e(\Hilb^k(\mathcal{C}/\Lambda))$ is the integral over $S^{[k]}$ of
% the coefficient of $\omega^{\delta}$ in the integrand above.


\step{}
We now end the proof with the recursion procedure developed in
\cite{EGL}, see Proposition~\ref{P:rec}. 
The latter, applied $k$ times, turns the above integral over
$\HS k$
%in \eqref{e(Hilb^k} 
into the integral over $S^k$ of a polynomial in the Chern classes 
of $\pr_i^*L$, $\pr_i^* T_S$, and $\pr_{ij} ^* T_\Delta$ ($i\neq j$), 
where $\Delta \subset S\times S$ is the diagonal, 
$\pr_i:S^k \to S$ is the $i$-th projection, and
$\pr_{ij} = (\pr_i,\pr_j)$.
The latter integral results
(with some non-trivial work, see, for instance,
\cite[Proposition 0.5 and its proof]{EGL})
in a polynomial in $L^2$, $LK_S$, $K^2_S$, and
$c_2(S)$, of degree at most $k$.

% To compute the degree of the universal polynomial we shall obtain, we
% need to prove that the integral \eqref{e(Hilb^k} is in fact a
% polynomial of degree exactly $k$  in $L^2$, $LK_S$, $K^2_S$, and
% $c_2(S)$. 
It remains to prove that this degree is exactly $k$.
To do so, we concentrate on the $c_2(S)^k$ term.
One looks the explicit formulas for the recursion straight in the eyes, 
viz.\ \eqref{rec:I}, \eqref{rec:II}, \eqref{rec:III}, \eqref{rec:IV}, 
\eqref{rec:8}, 
and finds that the only contribution to the $c_2(S)^k$ term comes
from the $c_0(L^{[k]})$ term.
One may thus, for our present purpose, replace the fraction in
\eqref{e(Hilb^k} by
\[
\frac
{c_\bullet(T_{S^{[k]}}) (1+\omega)^{\delta+1}
\omega^k}
{(1+\omega)^{k}}
= c_\bullet(T_{S^{[k]}})
\omega^k (1+\omega)^{\delta-k+1}, 
\]
the coefficient of which in $\omega^\delta$ is 
$(\delta-k+1)\, c_\bullet(T_{S^{[k]}})$.
The corresponding summand of the integral \eqref{e(Hilb^k} is
$(\delta-k+1)\,c_{2k}(T_{S^{[k]}})$, which contributes by
$(\delta-k+1)/k!$ to the $c_2(S)^k$ term, the factorial coming from
the $k$ successive applications of \eqref{rec:0}.
\end{proof}


\begin{example}
Let us spell out this computation for the number of $1$-nodal curves in
a pencil, and see how it relates with the standard way to do it, which
we recalled in the introduction to the present Section~\ref{section KST}.
In this case we have $\Lambda \simeq \P^1$. Equation \eqref{eq:ek_nv} gives
\[
e(\Hilb^1(\cC/\Lambda)) 
= n_{\Lambda,p-1} - (2p-2)n_{\Lambda,p}
\quad \text{and}
\quad
e(\Hilb^0(\cC/\Lambda)) =n_{\Lambda,p}.
\]
We have $e(\Hilb^0(\cC/\Lambda))=e(\Lambda)=2$, and we concentrate on the
computation of $e(\Hilb^1(\cC/\Lambda))$ as the integral \eqref{e(Hilb^k}. 
The numerator of the integrand of \eqref{e(Hilb^k-0} is
\begin{align*}
(1-K+c_2)(1+\omega)^2(L+\omega)
&=
(1-K+c_2)(1+2\omega)(L+\omega)
\\
% &= 
% (1-K+c_2)(L+(1+2L)\omega)
% \\
&=
\bigl[L-KL\bigr]+
\bigl[
1-K+2L+c_2-2KL
\bigr] \omega,
\end{align*}
and on the other hand
\begin{align*}
\frac 1
{1+L+\omega}
&= 1 -(L+\omega)+(L+\omega)^2-(L+\omega)^3
\\
&= 
1-(L+\omega)+(L^2+2L\omega)-3L^2\omega
=
\bigl[ 1-L+L^2 \bigl]
+ \bigr[ 
-1+2L-3L^2
\bigl] \omega.
\end{align*}
The coefficient in $\omega$ of the integrand of \eqref{e(Hilb^k-0}
is therefore
\begin{equation*}
(L-KL)
(-1+2L-3L^2)
+(1-K+2L+c_2-2KL)
(1-L+L^2)
=
1-K+L^2+c_2;
\end{equation*}
integrated against the
fundamental class $[S]$, it gives $L^2+c_2$, as required,
see \ref{p:KST-idea}.
\end{example}


\subsection{The Ellingsrud--G\"ottsche--Lehn recursion}
\label{s:EGL}

We now describe the inductive computation of \cite{EGL}.
Our aim is to provide the right amount of detail
so that: i) one may make sense of the arguments at the end of
the proof of Proposition~\ref{P:e(Hilb^k)};
and ii) one should be able to make it work in practice. 
We refer to the original article \cite{EGL} for the proofs.

Let $S$ be a smooth projective surface, equipped with a line bundle $L
\to S$. We consider the Hilbert schemes $\HS n$ and the vector bundles
$L^{[n]} \to \HS n$. We call $T_n$ the tangent sheaf of $\HS n$,
and $\I_n$ the ideal sheaf of the universal subscheme $Z_n
\subset \HS n \times S$.
For any sequence $I$ of indices in $\{0,\ldots,m\}$ we let $\pr_I$ be
the projection from $\HS {n} \times S^m
=\HS {n} \times S \times \cdots \times S$ 
to the
factors indexed by $I$, $\HS {n}$ being the $0$-th factor;
beware that we will (abusively) use this notation both for
$\HS {n+1} \times S^m$
and $\HS {n} \times S^{m+1}$.
We let $\Delta$ denote the diagonal in $S^2$.

\begin{proposition}
\label{P:rec}
Let $f$ be a polynomial in the Chern classes of the following sheaves
on $\HS {n+1} \times S^m$:
\[
\pr_0^* T_{n+1},\
\pr_{0i}^* \I_{n+1},\
\pr_{ij}^* \O_\Delta,\
\pr_i^* T_S,\
\pr_0^* L^{[n+1]},\
\pr_i^* L
\qquad
(\text{for}\
1 \leq i<j \leq m).
\]
There is a polynomial $f^\flat$
in the Chern classes of the analogously defined sheaves on 
$\HS {n} \times S^{m+1}$, depending only on $f$, and such that
\[
\int _{\HS {n+1} \times S^m} f
= \int_{\HS {n} \times S^{m+1}} f^\flat.
\]
\end{proposition}


Key to the recursive procedure is the consideration of the incidence
variety 
$\HS {n,n+1} \subset \HS n \times \HS {n+1}$ of all pairs $(Z,Z')$
such that $Z \subset Z'$. 
There is an identification 
$\HS {n,n+1} \cong \P(\I_n)$, coming from the fact that if $Z'$ is
obtained by extending $Z$ at the 
closed point $x\in S$, then the ideal sheaf defining $Z$ in $S$ is an
extension of the skyscraper sheaf $\C_x$ by the ideal sheaf of $Z'$.

We let $\cL=\O _{\P(\I_n)}(1)$.
and consider the following maps: $\phi$ and $\psi$ are the two projections
of $\P(\I_n)$ to $\HS n$ and $\HS {n+1}$, respectively, 
and $\rho: \P(\I_n) \to S$ 
maps a pair $(Z,Z')$ to the point $x\in S$ at which $Z$ and
$Z'$ differ.
\[\xymatrix@C=0mm{
& \kern 3mm \P(\I_n)=\HS {n,n+1} 
\ar[d]_\rho
\ar[dl]_(.6){\phi=\pr_1}
\ar[dr]^(.6){\psi=\pr_2}
\\
\HS n 
& S
& \HS {n+1}
}
\]
Moreover,
let $j=(\id,\rho):\P(\I_n) \to \P(\I_n)\times S$,
$\phi_S = \phi \times \id_S: \P(\I_n) \times S \to \HS n \times S$,
and $\psi_S = \psi \times \id_S: \P(\I_n) \times S \to \HS {n+1}
\times S$. 
We have the following exact sequence of sheaves on
$\HS {n,n+1} \times S$:
\begin{equation}
\label{eq:EGL5}
%\tag{5}
0 \to \psi_S^* \I_{n+1} \to \phi_S^* \I_n \to j_* \cL \to 0.
\end{equation}
Note that $j_* \cL = p^* \cL \otimes \rho_S ^* \O_\Delta$,
where $p$ is the projection $\HS {n,n+1} \times S \to \HS {n,n+1}$,
and $\rho_S=\rho\times \id_S: \HS {n,n+1} \times S \to S^2$.

\begin{proof}[Proof of Proposition~\ref{P:rec}]
We want to relate integrals on $\HS {n+1} \times S^m$ to integrals on
$\HS n \times S^{m+1}$.
To this end we consider the product $\Sigma= \HS {n,n+1} \times S^m$,
together with the maps
$\Psi= \psi \times \id_{S^m}: \Sigma \to \HS {n+1} \times S^m$
and $\Phi=(\phi,\rho)\times \id_{S^m}: \Sigma \to \HS n \times S \times
S^m$.
Moreover, we call $p_\Sigma: \Sigma=\HS {n,n+1} \times S^m \to \HS {n,n+1}$
the projection on the first factor.
\[
\xymatrix@C=0mm{
& \Sigma= \HS {n,n+1} \times S^m
\ar[dl]_(.55){\Psi=\psi\times \id}
\ar[dr]^(.55){\Phi=(\phi,\rho)\times \id}
\ar[d]_{p_\Sigma}
\\
\HS {n+1} \times S^m
& \HS {n,n+1}
& \HS n \times S \times S^m
}
\]

The first step is to lift our integral to $\Sigma$, using the fact that
$\Psi$ is generically finite of degree $n+1$. This gives:
\begin{equation}
\label{rec:0}
\int _{\HS {n+1} \times S^m} f
= \frac 1 {n+1}
\int _\Sigma \Psi^*f.
\end{equation}
We aim to find an expression for $\Psi^*f$ of the form
$\sum_{\nu \geq 0} \Phi^* f_\nu \cdot 
p_\Sigma^*\bigl( c_1(\cL)^\nu
\bigr)$,
in the Grothendieck ring $K(\Sigma)$ of coherent sheaves on $\Sigma$.
Then we will conclude by applying the projection formula.

We first have the following two straightforward formulas
(in the Grothendieck ring, as will be the case for all other formulas
of the same kind), which
display on 
simple instances the index shift resulting from the additional $S$ factor
induced by the $\rho$ component of $\Phi$.
\begin{align}
\label{rec:I}
\Psi^* \pr_i^* T_S 
&= \Phi^* \pr_{i+1}^* T_S
\\
\label{rec:II}
\Psi^* \pr_{ij}^* \O_\Delta
&= \Phi^* \pr_{i+1,j+1}^*  \O_\Delta.
\end{align}
Beware that, by abuse of notation,
the '$\pr$' on the left-hand-side refer to
projections from $\HS {n+1} \times S^m$ 
whereas those on the right-hand-side refer to
projections from $\HS {n} \times S^{m+1}$.
The first non-trivial formula in the induction procedure is the
following, and comes from \eqref{eq:EGL5} together with the given
expression for $j_*\cL$:\footnote
{note that there is a typo in the corresponding formula in
  \cite[Proof of Prop.~3.1]{EGL} (on top of p.~89):
  the '$+$' sign there should be a '$-$' sign;
this is the same ``small sign error'' that is hinted at on the very
last line of \cite{KST-12}, as was kindly indicated to us by Martijn Kool.}
\begin{equation}
\label{rec:III}
\Psi^* \pr_{0i} ^* \I_{n+1}
= \Phi^* \pr_{0,i+1} ^* \I _n
- p_\Sigma ^* \cL \cdot 
\Phi^* \pr_{1,i+1} ^* \O_\Delta.
\end{equation}
% (WARNING: $\pr_{0,i+1}$ in $\Phi$-term refers to (IMO) the projection 
% from $\HS n \times S^{m+1}$ instead of $\HS {n+1} \times S^m$).
% $p_\Sigma: \Sigma=\HS {n,n+1} \times S^m \to \HS {n,n+1}$.
% The last term comes (I guess) from the identification 
% $j_* \cL = p^* \cL \otimes \rho_S ^* \O_\Delta$.
Next we have the following relation, which is a consequence of the
computation in the Grothendieck group of $\HS {n,n+1}$ carried out in
\cite[\S 2]{EGL}:
\begin{multline}
\label{rec:IV}
\Psi^* \pr_0^* T_{n+1} 
\\= \Phi^* \pr_0^* T_n
+ p_\Sigma ^* \cL 
\cdot \Phi^* \pr_{01}^* \I_n ^\vee
+ p_\Sigma ^* \cL ^\vee
\cdot \Phi^* \pr_{01}^* \I_n
\cdot \Phi^* \pr_1 ^* \omega_S ^\vee
- \Phi^* \pr_1^* (\O_S - T_S + \omega_S ^\vee).
\end{multline}
The last relation follows from \cite[Lemma~2.1]{EGL}:
\begin{equation}
\label{rec:8}
\Psi^* \pr_0^* L^{[n+1]} = 
\Phi^* \pr_0^* L^{[n]}
+ p_\Sigma^* \cL \cdot \Phi^* \pr_1^* L.
\end{equation}

Now, applying formulas
\eqref{rec:I},
\eqref{rec:II},
\eqref{rec:III},
\eqref{rec:IV},
and \eqref{rec:8}
to transform $\Psi^* f$,
and plugging the result in \eqref{rec:0},
one obtains an identity of the form
\begin{equation}
\label{nu}
\int _{\HS {n+1} \times S^m} f
= \int _{\Sigma} 
\Bigl(
\sum\nolimits_{\nu \geq 0} \Phi^* f_\nu \cdot 
p_\Sigma^*\bigl( c_1(\cL)^\nu
\bigr)
\Bigr)
\end{equation}
as we wanted.
By the projection formula,
the right-hand-side equals
\begin{equation*}
\int _{\HS n \times S^{m+1}} 
\Phi_* \Bigl(
\sum\nolimits_{\nu \geq 0} \Phi^* f_\nu \cdot 
p_\Sigma^*\bigl( c_1(\cL)^\nu
\bigr)
\Bigr)
= \int _{\HS n \times S^{m+1}} 
\Bigl(
\sum\nolimits_{\nu \geq 0}
(-1)^\nu
f_\nu \cdot 
c_\nu(-\pr_{01}^* \I_n)
\Bigr),
\end{equation*}
where the last equality is given by the identity
$(\phi,\rho)_* \bigl( c_1(\cL)^\nu \bigr)
= (-1)^\nu c_\nu (-\I_n)$
in the Chow ring of $\HS n \times S$, see
\cite[Lemma~1.1]{EGL}.\footnote
{By definition the Chern classes $c_\nu(-\mathcal{F})$ are the
coefficients of the multiplicative inverse of the Chern polynomial
$c_t(\mathcal{F})$, 
\ie the Chern classes $c_\nu(-\mathcal{F})$ are the Segre classes
$s_\nu(\mathcal{F})$.}
% that is the formal power series
% $\sum_{\nu \geq 0} s_\nu(\mathcal{F})t^\nu$ with coefficients the
% Segre classes of $\mathcal{F}$.
This ends the proof.
\end{proof}

\begin{example}
To illustrate the recursion,
let us compute $\int_{\HS 2} c_2(L^{[2]})^2$.
We consider the diagram
\[
\xymatrix@C=0mm{
& \Sigma= \HS {1,2} \times \{\mathrm{pt}\}
\ar[dl]_{\Psi}
\ar[dr]^{\Phi}
\ar[d]_{p}
\\
\HS {2} \times  \{\mathrm{pt}\}
& \HS {1,2}
& \HS 1 \times S \times \{\mathrm{pt}\}
}
\]
in which $\{\mathrm{pt}\}$ denotes the point. This factor may of
course be forgotten, except for compatibility with the general
notation; thus, the map $p$ is merely the identity.
Also, the pair $(\HS 1, L^{[1]})$ may be identified with $(S,L)$.

We start from the identity
$\int_{\HS 2} c_2(L^{[2]})^2
= \frac 1 2 \int_{\HS {1,2}} \Psi^* c_2(L^{[2]})^2$.
Next, we have
$\Psi^* L^{[2]} = \Phi^* \pr_0^*L + p^*\cL\cdot \Phi^*\pr_1^*L$
by \eqref{rec:8}.
In general, $c_2(A+B) = c_2(A)+c_2(B)+c_1(A)c_1(B)$; here,
$\Psi^*L^{[2]}$ is expressed as a sum of line bundle, so we simply
have
\begin{equation*}
  c_2 (\Psi^* L^{[2]})
  = c_1(\Phi^* \pr_0L)
  \cdot
  \bigl(
  c_1(p^*\cL)+ c_1(\Phi^*\pr_1^*L)
  \bigr)
\end{equation*}
(we have also used that $c_1(AB)=c_1(A)+c_1(B)$),
hence
\begin{equation*}
  c_2 (\Psi^* L^{[2]})^2
  = \Phi^* \pr_0^* c_1(L)^2
  \cdot
  \bigl(\,
  \underbrace{p^*c_1(\cL)^2}_{\nu=2}+
  \underbrace{2 p^*c_1(\cL) \cdot \Phi^*\pr_1^*c_1(L)} _{\nu=1}
  + \underbrace{\Phi^*\pr_1^*c_1(L)^2} _{\nu=0}
  \,\bigr)
\end{equation*}
($\nu$ is the index that appears at the end of the proof of
Proposition~\ref{P:rec}, from \eqref{nu} on).

Now, the universal subscheme
$Z_1 \subset \HS 1 \times S$
identifies with the diagonal $\Delta$ in $S\times S$, and we thus have
$\O_{S\times S} = \cI_1 + \iota_* \O_\Delta$,
where $\iota$ denotes the inclusion map $\Delta \hookrightarrow
S\times S$.
Therefore,
$c_1(\cI_1) = -c_1(\iota_* \O_\Delta)$,
and $c_2(\cI_1) = -c_2(\iota_* \O_\Delta)$.
By the Riemann--Roch formula without denominators,
we have
\[
  c_1(\iota_* \O_\Delta) = 0
  \et
  c_2(\iota_* \O_\Delta) = -[\Delta],
\]
see \cite[Example 15.3.1]{F}.
Thus,
\[
  \frac 1 {1+c_1(\cI_1)+c_2(\cI_1)+\cdots}
  = \frac 1 {1+[\Delta]+\cdots}
  = 1 -[\Delta]+ \cdots,
\]
hence
\[
  \Phi_*p^* c_1(\cL) = -c_1 (-\cI_1) = 0
  \et
  \Phi_*p^* c_1(\cL)^2 = c_2 (-\cI_1) = -[\Delta].
\]
In the upshot,
\begin{gather*}
  \int_{\HS {1,2}}
  \Phi^* \pr_0^* c_1(L)^2
  \cdot
  \Phi^*\pr_1^*c_1(L)^2
  = \int_S c_1(L)^2\cdot \int_S c_1(L)^2
  = (L^2)^2,
  \\
  \int_{\HS {1,2}}
  \Phi^* \pr_0^* c_1(L)^2
  \cdot
  2 p^*c_1(\cL) \cdot \Phi^*\pr_1^*c_1(L)
  = -2 \int_{S\times S}
  \pr_0^* c_1(L)^2
  \cdot \pr_1^*c_1(L)
  \cdot c_1(-\cI_1)
  = 0,
  \\
  \int_{\HS {1,2}}
  \Phi^* \pr_0^* c_1(L)^2
  \cdot
  p^*c_1(\cL)^2
  = \int_{S\times S}
  \pr_0^* c_1(L)^2
  \cdot c_2(-\cI_1)
  = -\int_{S\times S}
  \pr_0^* c_1(L)^2
  \cdot [\Delta]
  = -L^2,
\end{gather*}
and therefore
\[
  \int_{\HS 2} c_2(L^{[2]})^2
  = \frac 1 2
  \int _{{\HS {1,2}}} \Psi^* c_2(L^{[2]})^2
  = \frac 1 2
  L^2(L^2-1).
\]
\end{example}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Tzeng's proof of the G\"ottsche--Yau--Zaslow formula}\label{section T}

In this section, we outline the proof
of Theorem \ref{theorem T} given by Tzeng \cite{T}.
The plan of the proof is the following. 
In \S \ref{sub cobordism}, we follow \cite{LeeP} in order to define the algebraic cobordism group $\left(\omega_{2,1},+\right)$ of equivalence classes of pairs $[S,L]$ of surfaces and line bundles with respect to the extended double point relation (\cf Definition \ref{def EDP}), endowed with the sum induced by disjoint union of surfaces. 
Then we recall the description of $\omega_{2,1}\otimes_{\Z}\Q$ as a four dimensional vector space over $\Q$ spanned by $[\P^2,\mathcal{O}_{\P^2}]$, $[\P^2,\mathcal{O}_{\P^2}(1)]$, $[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}]$, and $[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}(1,0)]$.

In \S \ref{sub Gottsche} we introduce G\"ottsche's enumerative
integrals $d_{\delta}(S,L)$ of a line bundle $L$ on a smooth surface
$S$, and we show,
following Göttsche,
that if $L$ is sufficiently ample, then  $d_{\delta}(S,L)$ equals the number $a_{\delta}(S,L)$ of $\delta$-nodal curves in a general $\delta$-dimensional linear subsystem of $|L|$.

Section \ref{sub degeneration} is dedicated to
Tzeng's degeneration formula for the numbers $d_{\delta}(S,L)$.
It can be understood as saying that the map
$\phi: (S,L) \mapsto \sum d_{\delta}(S,L)x^{\delta}$
is a homomorphism of $\Q$-vector spaces between the algebraic
cobordism group $\omega_{2,1}\otimes_{\Z}\Q$ and the space of
invertible power series $\left(\Q[[x]]^{\times},\cdot\right)$.

Finally, \S \ref{sub proofs} contains
the proofs of Theorems \ref{theorem G} and \ref{theorem T}. 
The proof of Theorem \ref{theorem G} mostly consists in putting
together the results of the previous sections;
after that, Theorem \ref{theorem T} is obtained by plugging in the Bryan--Leung
formula in addition.

% Thanks to the results of \S \ref{sub cobordism} and \S \ref{sub degeneration}, we prove the analogous of Theorem \ref{theorem G} for the generating function $\phi(S,L)$, by considering the decomposition of an arbitrary pair $[S,L]$ as a sum of copies of $[\P^2,\mathcal{O}_{\P^2}]$, $[\P^2,\mathcal{O}_{\P^2}(1)]$, $[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}]$, and $[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}(1,0)]$.
% Then the assertion of Theorem \ref{theorem G} for the generating function $T(S,L)$ of the numbers $a_{\delta}(S,L)$ follows from Theorem \ref{theorem KST} and the equality between $d_{\delta}(S,L)$ and $a_{\delta}(S,L)$ presented in \S \ref{sub Gottsche}.
% Finally, the G\"ottsche--Yau--Zaslow formula is proved by means of Theorem \ref{theorem G} and the Bryan--Leung formula \cite[Theorem 1.1]{BL-12},
% see \cite{10.th-panoramico}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{The algebraic cobordism group of surfaces and line bundles}\label{sub cobordism}

We now review the construction of the algebraic cobordism group
$\left(\omega_{2,1},+\right)$ of line bundles on surfaces,
and the results of \cite{LeeP} giving a basis of
$\omega_{2,1}\otimes_{\Z}\Q$ as a $\Q$-vector space.

Let $(\mathcal{M}_{2},+)$ denote the free abelian group generated by isomorphism classes $[S]$ of smooth projective surfaces.
One may think of the sum of two distinct isomorphism classes $[S_1]$ and $[S_2]$ in $\mathcal{M}_{2}$ as the isomorphism class of the disjoint union $S_1\sqcup S_2$.   

\begin{definition}\label{def DP}
We say that four smooth projective surfaces $S_0,\dots,S_3$ satisfy a \emph{double point relation} $[S_0]-[S_1]-[S_2]+[S_3]$ if there exists a family $\mathcal{X}\stackrel{\pi}{\longrightarrow} \P^1$ of surfaces such that:
\begin{compactitem}
  \item[(i)] the total space $\mathcal{X}$ is smooth of pure dimension 3;
  \item[(ii)] the fibre over $0$ is $S_0$;
  \item[(iii)]  $S_1$ and $S_2$ are smooth divisors of $\cX$
    intersecting transversely, and
    the fibre over $\infty$ is the union
    $S_1\cup S_2$;
  \item[(iv)] let $D=S_1\cap S_2$;
    the surface $S_3$ is the $\P^1$-bundle
    $\P(\mathcal{O}_{D}\oplus N_{D/S_1})\cong \P(N_{D/S_2}\oplus \mathcal{O}_{D})$.
\end{compactitem}
\end{definition}

\noindent
In the above, $N_{D/S}$ denotes the normal bundle of $D$ in $S$.
Note that the surfaces $S_1,S_2$ and the curve $D$ are allowed to
be disconnected and empty.

\begin{remark}
\label{rk:S_1S_2}
The isomorphism $\P(\mathcal{O}_{D}\oplus N_{D/S_1})\cong
\P(N_{D/S_2}\oplus \mathcal{O}_{D})$ in (iv) above follows from the
fact that $ \mathcal{O}_{D}(S_1+S_2)\cong \mathcal{O}_{D}$.
Indeed, it implies $N_{D/S_1}\otimes N_{D/S_2}\cong \mathcal{O}_{D}$,
hence 
$\mathcal{O}_{D}\oplus N_{D/S_1}\cong (N_{D/S_1}\otimes N_{D/S_2})\oplus (N_{D/S_1}\otimes \mathcal{O}_{D})\cong N_{D/S_1}\otimes (N_{D/S_2}\oplus\mathcal{O}_{D})$.
See also the discussion of the triple point formula and its variants in
\cite[Section \tref{s:setting}]{01.ciro}.
\end{remark}

Analogously,
let $(\mathcal{M}_{2,1},+)$
be the free abelian group generated by isomorphism classes $[S,L]$, where $S$ is a smooth projective surfaces and $L$ is a line bundle on $S$,
and extend Definition \ref{def DP} as follows.

\begin{definition}\label{def EDP}
For $i=0,\dots,3$, let $[S_i,L_i]$ be the class of a pair of a smooth projective surface $S_i$ and a line bundle $L_i$ on it.
We say that 
\begin{equation}\label{eq EDP}
[S_0,L_0]-[S_1,L_1]-[S_2,L_2]+[S_3,L_3]
\end{equation}
is an \emph{extended double point relation} if $[S_0]-[S_1]-[S_2]+[S_3]$ is a double point relation via a family $\mathcal{X}\stackrel{\pi}{\longrightarrow} \P^1$ of surfaces as above, and there exists a line bundle $\mathcal{L}$ on $\mathcal{X}$ such that $L_i=\mathcal{L}|_{S_i}$ for $i=0,1,2$,
and $L_3=\eta^*(\mathcal{L}|_{D})$, where $\eta$ is the structure map
\[
  \eta: S_3 = \P(\mathcal{O}_{D}\oplus N_{D/S_1})
  \longrightarrow D.
\]
\end{definition}

The following fundamental example is closely related to the
degeneration to the normal cone. For $\P^2$, it is the degeneration
to $\P^2 \cup_{\P^1} \F_1$
used in \cite{CH-12}, see \cite{04.concettina}.

\begin{example}[{see \cite[Lemma 2.4]{T}}]
\label{example blowup}
Let us consider a smooth projective surface $S$ and a line bundle $L$ on $S$. 
Given a smooth curve $C\subset S$, let $\mathcal{X}\stackrel{\mathrm{bl}}{\longrightarrow} S\times \P^1$ be the blow-up of the product $S\times \P^1$ along the curve $C\times \{\infty\}$, and let $E\cong\P(\mathcal{O}_{C}\oplus N_{S/C})$ be its exceptional divisor endowed with the $\P^1$-bundle map $E\stackrel{\eta}{\longrightarrow} C$. 
The following is an extended double point relation
for all integers $k$,
\[ 
\bigl[S,L\bigr]-\bigl[S,L(-kC)\bigr]-\bigl[E,\eta^*(L|_{C})\otimes \mathcal{O}_E(kC)\bigr]+\bigl[E,\eta^*L(-kC)|_{C})\bigr].
\]
% $$ 
% [S,L]-[S,L\otimes \mathcal{O}_S(-kC)]-[E,\eta^*(L|_{C})\otimes \mathcal{O}_E(kC)]+[E,\eta^*((\mathcal{O}_S(-kC)\otimes L)|_{C})].
% $$
To see this fact, let $\mathrm{pr}_1\colon S\times \P^1\to S$ and $\mathrm{pr}_2\colon S\times \P^1\to\P^1$ denote the natural projections.
Consider the family $\mathcal{X}\stackrel{\mathrm{\pi}}{\longrightarrow} \P^1$ given by $\pi:=\mathrm{pr}_2\circ \mathrm{bl}$, and define a line bundle $\mathcal{L}$ on $\mathcal{X}$ as
$$
\mathcal{L}:= (\mathrm{bl}^*\mathrm{pr}_1^*L)\otimes \mathcal{O}_{\mathcal{X}}(-kC). 
$$ 
The morphism $\pi$ is a smooth over $\P^1-\{\infty\}$,
with fibres $\pi^{-1}(0)\cong S$ and
$\pi^{-1}(\infty) \cong S\cup_C E$.
Finally, defining $S_0,S_1\cong S$ and $S_2,S_3\cong E$ as in Definition \ref{def DP}, the line bundle $\mathcal{L}$ is such that $\mathcal{L}|_{S_0}= L$, $\mathcal{L}|_{S_1}= L\otimes \mathcal{O}_S(-kC)$, $\mathcal{L}|_{S_2}= \eta^*(L|_{C})\otimes \mathcal{O}_E(kC)$, and $\mathcal{L}|_{S_3}= \eta^*((\mathcal{O}_S(-kC)\otimes L)|_{C})$.
\end{example}

\noindent
We may now define the algebraic cobordism group of line bundles on surfaces.

\begin{definition}
Let $\mathcal{R}$ denote the subgroup of $\mathcal{M}_{2,1}$ generated by all extended double point relations. 
The \emph{algebraic cobordism group} of surfaces and line bundles is
the quotient
$$
\omega_{2,1}:=\mathcal{M}_{2,1}/\mathcal{R}.
$$
\end{definition}  

One may define more generally the
algebraic cobordism group
$\omega_{n,r}$ of isomorphism classes of pairs of $n$-dimensional varieties and rank $r$-vector bundles.
Lee and Pandharipande \cite{LeeP} described the structure of the $\Q$-vector space $\omega_{n,r}\otimes_{\Z} \Q$, by exhibiting a basis and showing that Chern invariants respect algebraic cobordism.  
In the case of surfaces and line bundles, \cite[Theorems 1 and 4]{LeeP}
give the following,
% obtained by Tzeng independently,
see \cite[Theorem 2.3]{T}.

\begin{theorem}\label{theorem T2.3}
The map
$[S,L]\mapsto (L^2,LK_S,K_S^2,c_2(S))$
is an isomorphism $\omega_{2,1}\otimes_{\Z} \Q\cong \Q^4$
of $\Q$-vector spaces.
The family
\begin{equation}\label{eq basis}
  \left(\,
    [\P^2,\mathcal{O}_{\P^2}],\
    [\P^2,\mathcal{O}_{\P^2}(1)],\
    [\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}],\ [\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}(1,0)]
  \,\right)
\end{equation}
is a basis of the vector space $\omega_{2,1}\otimes_{\Z} \Q$, and for any pair $[S,L]$, we have
$$
\bigl[S,L\bigr]=a_1\bigl[\P^2,\mathcal{O}_{\P^2}\bigr]+ a_2\bigl[\P^2,\mathcal{O}_{\P^2}(1)\bigr]+ a_3\bigl[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}\bigr]+a_4\bigl[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}(1,0)\bigr],
$$
with ${a_1=-L^2+\frac{K_S^2-2c_2(S)}{3}}$, ${a_2=L^2}$, ${a_3=\frac{3L^2+LK_s}{2}-\frac{K_S^2-3c_2(S)}{4}}$ and ${a_4=-\frac{3L^2+LK_S}{2}}$.
\end{theorem}

%\begin{proof}
The first assertion is the content of
\cite[Theorems 1 and 4]{LeeP}, the proof of which we will not
discuss. A fundamental input behind it is
\cite[Theorem 1.2.19]{levine-morel}.

This being established,
proving that the family in \eqref{eq basis} is a basis is elementary:
it is enough to check that the 4-tuples
$(L^2,LK_S,K_S^2,c_2(S))\in \Q^4$
corresponding to the basis vectors 
are linearly independent,
which may be seen by computing them explicitly;
one finds $(0,0,9,3)$, $(1,-3,9,3)$, $(0,0,8,4)$, and $(0,-2,8,4)$,
respectively.
Then, one obtains the values of $a_1,\dots,a_4$ for
$[S,L]$ by solving for them in
the equality $(L^2,LK_S,K_S^2,c_2(S))=a_1(0,0,9,3)+\dots+a_4(0,-2,8,4)$.
%\end{proof}


\begin{remark}\label{remark basis}
For future use, note
that a family
$([S_i,L_i])_{i=1,\dots,4}$ gives a basis of
$\omega_{2,1}\otimes_{\Z} \Q$ if and only if the corresponding vectors $(L_i^2,L_iK_{S_i},K_{S_i}^2,c_2(S_i))\in \Q^4$ are linearly independent over $\Q$.
\end{remark}

\begin{remark}\label{remark 4tuples}
  Note that the data of the 4-tuples $(L^2,LK_S,K_S^2,c_2(S))$ and $(\chi(L),LK_S,K_S^2,\chi(\mathcal{O}_S))$ are equivalent since,
  by Noether's formula and the Riemann--Roch theorem, 
$$
\chi(\mathcal{O}_S)=\frac{1}{12}\left(K_S^2+c_2(S)\right)\quad \textrm{and}\quad \chi(L)=\chi(\mathcal{O}_S)+\frac{1}{2}\left(L^2-LK_S\right).
$$
% Thus we may define another isomorphism $\omega_{2,1}\otimes_{\Z} \Q\cong \Q^4$ by $[S,L]\longmapsto (\chi(L),LK_S,K_S^2,\chi(\mathcal{O}_S))$.
% Besides, a set $\{[S_i,L_i]|i=1,\dots,4\}\subset \omega_{2,1}$ is a basis for $\omega_{2,1}\otimes_{\Z} \Q$ if and only if the corresponding vectors $(\chi(L_i),L_iK_{S_i},K_{S_i}^2,\chi(\mathcal{O}_{S_i}))\in \Q^4$ are linearly independent.\\
Observe moreover that the above formulas ensure that  $L^2-LK_S$ is even and $K_S^2+c_2(S)$ is divisible by 3 and 4, so that the coefficients $a_1,\ldots,a_4$ in Theorem \ref{theorem T2.3} turn out to be integers, as expected.
\end{remark}

\begin{example}
Let $[S_1,L_1]$ and $[S_2,L_2]$ be two classes consisting of a $K3$ surface endowed with a primitive line bundle. 
Then the 4-tuples $((\chi(L),LK_S,K_S^2,\chi(\mathcal{O}_S))$ corresponding to the family
\begin{equation}\label{eq basis2}
  \left(\, [\P^2,\mathcal{O}_{\P^2}],\ [\P^2,\mathcal{O}_{\P^2}(1)],\ [S_1,L_1],\ [S_2,L_2]
  \,\right)
\end{equation}
are $(1,0,9,1)$, $(3,-3,9,1)$, $\bigl(2+\frac{L_1^2}{2},0,0,2\bigr)$ and $\bigl(2+\frac{L_2^2}{2},0,0,2\bigr)$.
This implies that the family in \eqref{eq basis2} is a basis of $\omega_{2,1}\otimes_{\Z} \Q$ if and only if $L_1^2\neq L_2^2$.  
\end{example}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{G\"ottsche's enumerative integrals}\label{sub Gottsche}

In this section we introduce, following Göttsche \cite[Section 5]{G},
some intersection numbers
$d_{\delta}(S,L)$
on Hilbert schemes of points on $S$ which will be used as a substitute
for the numbers $a_{\delta}(S,L)$ of $\delta$-nodal curves in
a general $\delta$-dimensional linear subsystem of $|L|$;
this is
possible thanks to Theorem \ref{theorem G5.2}, due to Göttsche
as well,
which asserts that $a_{\delta}(S,L)$ and $d_{\delta}(S,L)$ coincide if
$L$ is sufficiently positive.

This substitution circumvents the issue that the numbers
$a_{\delta}(S,L)$ behave rather poorly under degeneration.
For instance,
we have seen in the first chapters of this volume, \eg
\cite{01.ciro}
and
\cite{04.concettina},
that in a degeneration of $S$ to a transverse union of two surfaces
$S_1$ and $S_2$,
in order to find the number $a_{\delta}(S,L)$ on $S_1 \cup S_2$ one
ought to count
not only  curves with nodes on $S_1$ and $S_2$,
but also curves with tacnodes along the double curve
$S_1 \cap S_2$.
In contrast, Tzeng's results presented in the next section establish
good properties of the numbers $d_{\delta}(S,L)$.

\medskip
For any integer $k>0$, let us consider the Hilbert scheme $S^{[k]}$ parameterizing $0$-dimensional subschemes of $S$ of length $k$, and let $Z_{k}\subset S\times S^{[k]}$ be the universal subscheme, with projections $\pi_1\colon Z_k\to S$ and $\pi_2\colon Z_k\to S^{[k]}$.
As in \S \ref{sub tautological}, we denote by $L^{[k]}$ the vector bundle of rank $k$ on $S^{[k]}$ given by $L^{[k]}:={\pi_2}_*{\pi_1}^*L$. 

\begin{definition}[G\"ottsche's enumerative integrals]
\label{def W}
  % [{G\"ottsche's enumerative integrals
  % \cite[Definition 5.1]{G}}]
Let $\mathring{W}^{3\delta}\subset S^{[3\delta]}$ be the locally closed subset 
parametrizing all closed subchemes of the form
$\coprod_{i=1}^\delta \Spec(\mathcal{O}_{S,x_i}/\mathfrak{m}^2_{S,x_i})$,
where
$x_1,\dots,x_{\delta}$ are pairwise distinct points of $S$.
% $$
% \biggl\{  \coprod_{i=1}^{\delta}\Spec\left(\mathcal{O}_{S,x_i}/\mathfrak{m}^2_{S,x_i}\right): x_1,\dots,x_{\delta}\in S\textrm{ are distinct}
% \biggr\},
% $$
Let $W^{3\delta}\subset S^{[3\delta]}$ be the closure of
$\mathring{W}^{3\delta}$;
it is birational to $S^{[\delta]}$.
We let
$$
d_{\delta}(S,L):=\int_{W^{3\delta}}c_{2\delta}(L^{[3\delta]}),
$$ 
and write the associated generating function
$$
\phi(S,L):=\sum_{\delta\geqslant 0}d_{\delta}(S,L)x^{\delta}.
$$
\end{definition}

In \cite[Proposition 5.2]{G}, G\"ottsche proved that if $L$ is
sufficiently ample with respect to $\delta$, then the number
$d_{\delta}(S,L)$ coincides with the number $a_{\delta}(S,L)$ of
$\delta$-nodal curves in a general $\delta$-dimensional linear
subsystem of $|L|$.
Having now Theorem \ref{theorem KST2.1} at hand, we can slightly
weaken the positivity condition and simplify the proof.

\begin{theorem}\label{theorem G5.2}
Let $S$ be a smooth projective surface,
and let $L$ be a $(3\delta-1)$-very ample line bundle on $S$, for some $\delta>0$.
Then a general linear subsystem of
$|L|$ of dimension $\delta$ contains exactly $d_{\delta}(S,L)$ curves having exactly $\delta$ nodes as singularities, \ie
$a_{\delta}(S,L)=d_{\delta}(S,L)$.
\end{theorem}

\begin{proof}
We will prove 
that a general linear subsystem $\Lambda\subset |L|$ of dimension
$\delta$ contains $d_{\delta}(S,L)$ curves
(counted with multiplicities)
having at least $\delta$ singularities.
Then, the result will follow directly from
Theorem \ref{theorem KST2.1},
see Remark \ref{rk:thm-KST2.1}.

Let $(s_1,\dots,s_{\delta+1})$  be a basis of the linear subspace
of $H^0(S,L)$ corresponding to $\Lambda\subset \P(H^0(S,L))$, and
consider the global sections
${\pi_2}_* \pi_1^*s_1, \ldots, {\pi_2}_*\pi_1^*s_{\delta+1}$
of the vector bundle $L^{[3\delta]}$.
Moreover, let $Y\subset S^{[3\delta]}$ be the locus of points
$[Z]\in S^{[3\delta]}$ such that the vectors
${\pi_2}_*{\pi_1}^*s_1(Z),\ldots,{\pi_2}_*{\pi_1}^*s_{\delta+1}(Z)$
are linearly dependent, \ie
such that there exists a divisor $D$ belonging to $\Lambda$ that
contains $Z$.

Since $L$ is $(3\delta-1)$-very ample,
the restriction map $H^0(S,L)\rightarrow H^0(Z, L\otimes \mathcal{O}_Z)$ is surjective for all $[Z]\in S^{[3\delta]}$, hence
the evaluation map
${H^0(S,L)\otimes \mathcal{O}_{S^{[3\delta]}}\rightarrow
  L^{[3\delta]}}$ is surjective as well,
and $L^{[3\delta]}$ is globally generated.
Thus, by \cite[Example 14.3.2]{F} applied to the restriction of
$L^{[3\delta]}$ to $W^{3\delta}$, we find that
$Y\cap W^{3\delta}$ has codimension $2\delta$ in
$W^{3\delta}$, and class
$[Y\cap W^{3\delta}]=c_{2\delta}(L^{[3\delta]})\cap [W^{3\delta}]$
by the Thom--Porteous formula.
Moreover, since the dimension of $W^{3\delta}\setminus \mathring{W}^{3\delta}$
is smaller than $2\delta$, the same argument applied to 
the restriction of $L^{[3\delta]}$ to
$W^{3\delta}\setminus \mathring{W}^{3\delta}$ gives that 
$Y\cap W^{3\delta}$ lies entirely in $\mathring{W}^{3\delta}$.

We conclude that 
the number of members of $\Lambda$
(counted with multiplicities)
containing a point of
$\mathring{W}^{3\delta}$
is
$d_{\delta}(S,L):=\int_{W^{3\delta}}c_{2\delta}(L^{[3\delta]})$. 
Now a curve $C\subset S$ contains a scheme $Z\in \mathring{W}^{3\delta}$
with $Z_\red = x_1+\cdots+x_\delta$
if and only if it
is singular at all points $x_1,\dots,x_{\delta}\in S$.
Therefore,
the number of curves in $\Lambda$ having at least $\delta$ singularities
is $d_{\delta}(S,L)$, and this ends the proof.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Degeneration of enumerative integrals}\label{sub degeneration}
We now follow \cite[Section 3]{T} in order to show how the generating
function $\phi(S,L)=\sum d_{\delta}(S,L)x^{\delta}$ of the G\"ottsche
enumerative integrals of a pair $(S,L)$
respects extended double point relations.
The result below is Tzeng's main contribution to the proof of the Göttsche
conjecture.
It rests on Proposition \ref{proposition T3.9}, which may be seen as a
version of Jun Li's celebrated degeneration formula
\cite{li-jdg}.

% can be determined from
% generating functions $\phi(S_1,L_1)$, $\phi(S_2,L_2)$ and
% $\phi(S_3,L_3)$, provided
% $[S,L]-[S_1,L_1]-[S_2,L_2]+[S_3,L_3]$ is an in $\mathcal{M}_{2,1}$. 
% More precisely, we outline the proof of the following (see \cite[Theorem 3.2]{T}).

\begin{theorem}\label{theorem T3.2}
If $[S_0,L_0]-[S_1,L_1]-[S_2,L_2]+[S_3,L_3]$ is an extended double point relation in $\mathcal{M}_{2,1}$, then
$$
\phi(S_0,L_0)=\frac{\phi(S_1,L_1)\phi(S_2,L_2)}{\phi(S_3,L_3)}.
$$
Equivalently, the map $\phi\colon
\bigl(
\omega_{2,1}\otimes_{\Z}\Q, +
\bigr)
\longrightarrow
\bigl( \Q[[x]]^{\times},\times \bigr)$
% induced by $[S,L]\longmapsto \phi(S,L)$
is a $\Q$-linear group homomorphism.
\end{theorem}

Let us consider a
family $\mathcal{X}\stackrel{\pi}{\longrightarrow} \P^1$ of surfaces
and a line bundle $\cL$
inducing the extended double point relation
$[S_0,L_0]-[S_1,L_1]-[S_2,L_2]+[S_3,L_3]$ appearing in the statement,
in the same notation as in Definitions \ref{def DP} and \ref{def EDP}.
For all $t\in \P^1$, we let $X_t$ be the fibre
$\pi^{-1}(t)$.
The fibre ${X}_0$ is $S_0$, and the fibre ${X}_\infty$
is the union of $S_1$ and $S_2$ meeting transversally along a smooth
curve $D$.

Let $\delta$ be a positive integer;
for all smooth surfaces $S$
we let $W_{S}^{3\delta} \subset  S^{[3\delta]}$
be as in Definition \ref{def W}.
% \ie the closure of the locus parametrizing subschemes
% $\coprod_{i=1}^\delta \Spec(\mathcal{O}_{S,x_i}/\mathfrak{m}^2_{S,x_i})$
% supported at $\delta$ distinct points.
The strategy of \cite{T} to prove Theorem \ref{theorem T3.2} is to
study the degeneration of $W_{X_t}^{3\delta}$ at $t=\infty$
by means of the good degeneration of Hilbert schemes constructed by
Li and Wu \cite{LW}, see also \cite[Section 3.4]{li-handbook}.

Let $U\subset \P^1$ be the largest open subset containing 
$\infty$ and such that $\pi$ is smooth over
$U -\{\infty\}$,
and let us still denote by $\mathcal{X}\stackrel{\pi}{\longrightarrow}
U$ the pullback of the original family over $\P^1$.
For all $n\geq 1$, Li and Wu construct
a family $\pi^{[n]}\colon \mathcal{X}^{[n]}\to U$
which is a proper and separated Deligne--Mumford stack of finite type over $U$,
such that for all $t\neq \infty$, the fibre of
$\mathcal{X}^{[n]}$
over $t$ is the Hilbert scheme ${X}^{[n]}_t$ of $n$ points on
the smooth surface ${X}_t$; the fibre over $\infty$ is
different, however, as we will see.

The first step in the construction is to replace
$\mathcal{X}\stackrel{\pi}{\longrightarrow} U$ by an alternative
family
$\pi[n]\colon\mathcal{X}[n]\to U$ of surfaces,
called an \emph{expansion},
equal to $\cX \to U$ over $U-\{\infty\}$,
and with fibre over $\infty$ a semistable model
of $S_1\cup S_2$, viz.\
$$
\mathcal{X}[n]_{\infty}:=S_1\cup \Delta_1\cup \Delta_2\cup\dots\cup\Delta_{n-1}\cup S_2
$$
where,
for all $i=1,\ldots, n-1$, the surface
$\Delta_i$ is a $\P^1$-bundle
$\P(\mathcal{O}_{D}\oplus N_{S_1/D})$
over $D$ with two distinguished sections $D_i^-$ and $D_i^+$, and $\mathcal{X}[n]_{\infty}$ is obtained by identifying $D_i^+\subset \Delta_i$ with $D_{i+1}^-\subset \Delta_{i+1}$, $D\subset S_1$ with $D_1^-\subset \Delta_1$, and $D_{n-1}^+\subset \Delta_{n-1}$ with $D\subset S_2$. 

Li and Wu introduce the notion of \emph{stable ideal sheaves},
see \cite[Definition 3.53]{li-handbook},
and let
$\pi^{[n]}\colon \mathcal{X}^{[n]}\to U$
be the moduli space of
stable ideal sheaves of the family $\mathcal{X}[n]\to U$.
For all $t\neq \infty$,
the fibre
${\pi^{[n]}}^{-1}(t)$ is the Hilbert scheme ${X}_t^{[n]}$
parametrizing $0$-dimensional subschemes of ${X}_t$ of length
$n$, whereas the fibre
${\pi^{[n]}}^{-1}(\infty)$ is the union
\begin{equation}\label{eq infty^[n]}
  \mathcal{X}_{\infty}^{[n]}:=\bigcup_{k=0}^n
  \bigl((S_1/D)^{[k]}\times(S_2/D)^{[n-k]}\bigr),
\end{equation}
where
$(S_1/D)^{[k]}$
(resp.\ $(S_2/D)^{[k]}$)
parametrizes
$0$-dimensional schemes of length $k$ supported on the smooth locus of
$S_1\cup \Delta_1\cup\dots\cup\Delta_{i}$
for some $i \leq k$
(resp.\ $\Delta_j\cup\dots\cup\Delta_{n-1}\cup S_2$
for some $j \leq n-k$);\footnote
{For a subscheme $Z$ supported on $S_1\cup
  \Delta_1\cup\dots\cup\Delta_{i}$
  (resp.\ $\Delta_j\cup\dots\cup\Delta_{n-1}\cup S_2$),
  we require moreover
  that all components $\Delta_1,\ldots,\Delta_{i}$
  (resp.\ $\Delta_j, \ldots, \Delta_{n-1}$)
  contain a point of the support of $Z$
  (the components not supporting any piece of $Z$ ought to be
  contracted).}
by convention,
$(S_1/D)^{[0]} = (S_2/D)^{[0]} = \{\textrm{pt}\}$.

We now set $n=3\delta$,
and consider
the expanded family of surfaces
$\pi{[3\delta]}\colon \mathcal{X}{[3\delta]} \rightarrow U$,
and
the moduli space of stable ideal sheaves
% the family of Hilbert schemes
$\pi^{[3\delta]}\colon \mathcal{X}^{[3\delta]}\rightarrow U$.\footnote
{beware the unfortunate proximity of the two otherwise standard
  notations.} 
The following lemma describes the good degeneration of
$W^{3\delta} _{X_t}$ in $\cX^{[3\delta]}$ at $t=\infty$.
Let $\mathcal{W}^{3\delta}$
be the the closure in $\mathcal{X}^{[3\delta]}$ of the set
\[
\mathring{\mathcal{W}}^{3\delta}
:=
\coprod_{t\neq \infty} \mathring{W}^{3\delta} _{X_t}
=\bigg\{
\Big[
\coprod_{i=1}^{\delta}
\Spec\left(\mathcal{O}_{{X}_t,x_i}/\mathfrak{m}^2_{x_i}\right)
\Big]:\,
\text{$t\neq \infty$ and $x_1,\dots,x_{\delta}\in {X}_t$
  pairwise distinct} \bigg\}.
\]
For all $k=1,\ldots,\delta$ and $i=1,2$, we let
$W_{S_i/D}^{3k}$ be the closure in $(S_i/D)^{[3k]}$ of the locus
parametrizing unions of $k$ disjoint subschemes of the form
$\Spec(\O_x/\fm_x^2)$;
by convention, $W_{S_i/D}^{0}:= \{\mathrm{pt}\}$.


\begin{lemma}[{\cite[Lemma 3.8]{T}}]
\label{lemma T3.8}
The map $\mathcal{W}^{3\delta}\rightarrow U$
is flat,
% family such that
% $$
% \mathcal{W}^{3\delta}\cap S_0^{[3\delta]}=W_{S_0}^{3\delta}
% $$
its fibre over $t\neq \infty$ is
$W^{3\delta} _{X_t}$,
and its fibre over $\infty$ is such that
for all $m=0,\ldots,3\delta$,
$$
\mathcal{W}^{3\delta}\cap
\big((S_1/D)^{[m]}\times (S_2/D)^{[3\delta-m]}\big)
=\left\{\begin{array}{ll}
W_{S_1/D}^{3k}\times W_{S_2/D}^{3(\delta-k)} &
\text{if $m=3k$ for some $k\in \mathbf{N}$} \\
\emptyset & \text{otherwise}.
\end{array}\right.
$$
\end{lemma}


Let us now briefly survey the definitions
of a universal subscheme over $\cX^{[n]}$, and
of a vector bundle
$\cL^{[n]}$ on $\cX^{[n]}$ from the line bundle $\cL$ on $\cX$,
see \cite[Definition-Proposition 3.4]{T}.
Let $n$ be a positive integer.
We consider the universal closed subscheme $Z_0^{[n]}\subset S_0\times S_0^{[n]}$.
For $i=1,2$ and $0\leqslant k\leqslant n$, we may also introduce
universal closed subschemes $Z_i^{[k]}\subset
(S_i/D)\times(S_i/D)^{[k]}$;
beware that $S_i/D$ denotes a suitable expansion of $S_i$ along the
curve $D$.
Let
$$
\xymatrix{Z_0^{[n]} \ar[d]_{p_0^{[n]}}\ar[r]^{q_0^{[n]}} & S_0^{[n]} \\ S_0 & }
\quad\text{and}\quad 
\xymatrix{Z_i^{[k]} \ar[d]_{p_i^{[k]}}\ar[r]^{q_i^{[k]}} & (S_i/D)^{[k]} \\ (S_i/D) & }
$$
be the corresponding projections, and define the vector bundles of
rank $3k$ 
$$
L_i^{[k]}:=(q_i^{[k]})_*(p_i^{[k]})^*L.
$$
for all $i=0,1,2$.
We denote by  $\pi_1^{[k,n]}$ and $\pi_2^{[k,n]}$ the natural projections
$$
\xymatrix{(S_1/D)^{[k]}\times(S_2/D)^{[n-k]} \ar[d]_{\pi_1^{[k,n]}}\ar[r]^-{\pi_2^{[k,n]}} & (S_2/D)^{[n-k]} \\ (S_1/D)^{[k]}. & }
$$
With this notation, there exists a universal closed subscheme $\mathcal{Z}\subset \mathcal{X}[n]\times \mathcal{X}^{[n]}$ with projections
$$
\xymatrix{\mathcal{Z} \ar[d]_{P}\ar[r]^{Q} & \mathcal{X}^{[n]} \\ \mathcal{X}[n]. & }
$$
Its fibres over $0$ and $\infty$ are $Z_0^{[n]}$ and
$$
\mathcal{Z}_{\infty}:=
\biggl(\bigcup_{k=0}^n \left( Z_1^{[k]}\times
  (S_2/D)^{[n-k]}\right)\biggr)
\cup \biggl(\bigcup_{k=0}^n \left((S_1/D)^{[k]}\times Z_2^{[n-k]} \right)\biggr),
$$
respectively.

There is a line bundle $\cL[n]$ on $\cX[n]$ obtained by pull-back from
the line bundle $\cL$ on $\cX$.
Setting $\mathcal{L}^{[n]}:=Q_*P^*\mathcal{L}[n]$, the following holds.
\begin{lemma}[{\cite[Lemmas 3.6 and 3.7]{T}}]
\label{lemma T3.6}
The sheaf $\mathcal{L}^{[n]}$ is a vector bundle of rank $3n$ over $\mathcal{X}^{[n]}$, such that 
$$
\mathcal{L}^{[n]}|_{S_0} = L_0^{[n]}
\quad \text{and}\quad \mathcal{L}^{[n]}|_{(S_1/D)^{[k]}\times (S_2/D)^{[n-k]}}=(\pi_1^{[k,n]})^*L_1^{[k]}\oplus (\pi_2^{[k,n]})^*L_2^{[n-k]}.
$$
\end{lemma}

\smallskip
In order to study degenerations of the G\"ottsche enumerative numbers,
we define for $i=1,2$ the \emph{relative Göttsche integrals} 
$$
d_k(S_i/D,L_i)=\left\{\begin{array}{ll}1 & \text{for }k=0 \\ \displaystyle\int_{W^{3k}_{S_i/D}}c_{2k}(L_i^{[3k]}) & \text{for }k\geqslant 1,\end{array}\right.
$$
and their \emph{relative generating function}
$$
\phi(S_i/D,L_i)=\sum_{k\geqslant 0}d_k(S_i/D,L_i)x^k.
$$
Note that the relative Göttsche integrals are defined independently of
the family $\cX\to U$, and depend only on $S_i$ and $D\subset
S_i$: to define $(S_i/D)^{[3k]}$ and $L_i^{[3k]}$, one considers the
degeneration to the normal cone as in Example \ref{example blowup}.

We may now finally state the degeneration formula which lies at the
heart of Tzeng's proof of the Göttsche conjecture.

\begin{proposition}[{\cite[Proposition 3.9]{T}}]
\label{proposition T3.9}
If $[S_0,L_0]-[S_1,L_1]-[S_2,L_2]+[S_3,L_3]$ is an extended double point relation in $\mathcal{M}_{2,1}$, then
\begin{equation}
\label{eq:Tz-degen-formula-0}
d_{\delta}\left(S_0,L_0\right)=\sum_{k=0}^{\delta}d_{k}\left(S_1/D,L_1\right)d_{\delta-k}\left(S_2/D,L_2\right),
\end{equation}
hence
\begin{equation}
\label{eq:Tz-degen-formula}
  \phi(S_0,L_0)=\phi(S_1/D,L_1)\cdot\phi(S_2/D,L_2).
\end{equation}
\end{proposition}

We emphasize that while $d_\delta(S_0,L_0)$ is a genuine Göttsche
integral, as defined in Section \ref{sub Gottsche},
the $d_k(S_i/D,L_i)$ are relative,
\ie they are defined in terms of good degenerations à la Jun Li et al.

\begin{proof}
Formula \eqref{eq:Tz-degen-formula-0}
follows from the good degeneration results surveyed above,
after fairly mechanical computations.
The moduli space of stable ideal sheaves
$\cX^{[3\delta]}\to U$
provides a degeneration of the Hilbert scheme $S_0^{[3\delta]}$ to a
moduli space defined on an expansion of $S_1 \cup _D S_2$,
see \eqref{eq infty^[n]}.
Within this degeneration,
the family $\cW^{3\delta} \to U$ provides a flat degeneration of
$W_{S_0}^{3\delta}$ to the fibre
$\cW^{3\delta}_\infty$ over $\infty \in U$,
see Lemma \ref{lemma T3.8},
and the vector bundle $\cL^{[3\delta]}$ provides a degeneration of
$L_0^{[3\delta]}$, see Lemma \ref{lemma T3.6}.
Formula \eqref{eq:Tz-degen-formula-0}
will follow from the equality
\begin{equation*}
  % \label{eq c_2}
c_{2\delta}(\mathcal{L}^{[3\delta]})
\bigl[\mathcal{W}^{[3\delta]}_0\bigr]
=c_{2\delta}(\mathcal{L}^{[3\delta]})
\bigl[\mathcal{W}^{[3\delta]}_\infty\bigr]:
\end{equation*}
the left-hand-side plainly writes 
\begin{equation*}
%\label{eq c_2_1}
  c_{2\delta}(\mathcal{L}^{[3\delta]})
  \bigl[\mathcal{W}^{[3\delta]}_0\bigr]
=c_{2\delta}(\mathcal{L}^{[3\delta]})\bigl[W^{[3\delta]}_{S_0}\bigr]
=\int_{W_{S_0}^{3\delta}}c_{2\delta}(L_0^{[3\delta]})
=d_{\delta}(S_0,L_0),
\end{equation*}
and we will see that the right-hand-side equals the right-hand-side of
\eqref{eq:Tz-degen-formula-0}, which will end the proof.

By Lemmas \ref{lemma T3.8}
and \ref{lemma T3.6}, we have
\begin{align*}
\notag
  c_{2\delta}(\mathcal{L}^{[3\delta]})
  \bigl[\mathcal{W}^{[3\delta]}_{\infty} \bigr] &
=c_{2\delta}(\mathcal{L}^{[3\delta]})\,
\Bigl[\,\bigcup\nolimits_{k=0}^{\delta}W_{S_1/D}^{3k}\times W_{S_2/D}^{3(\delta-k)} \,\Bigr]
   \\
%  \label{eq c_2_2}
&  =\sum_{k=0}^{\delta}c_{2\delta}\bigl(\,
(\pi_1^{[3k,3\delta]})^*L_1^{[3k]}\oplus
(\pi_2^{[3k,3\delta]})^*L_2^{[3(\delta-k)]}
\,\bigr)
\,
\bigl[W_{S_1/D}^{3k}\times W_{S_2/D}^{3(\delta-k)} \bigr].
\end{align*}
Now,
$$
c_{2\delta}\bigl(\displaystyle(\pi_1^{[3k,3\delta]})^*L_1^{[3k]}\oplus
  (\pi_2^{[3k,3\delta]})^*L_2^{[3(\delta-k)]}\bigr)
=\sum_{l=0}^{2\delta}c_l\bigl( (\pi_1^{[3k,3\delta]})^*L_1^{[3k]} \bigr)c_{2\delta-l}\bigl( (\pi_2^{[3k,3\delta]})^*L_2^{[3(\delta-k)]} \bigr),
$$
so that after capping with
$\bigl[W_{S_1/D}^{3k}\times W_{S_2/D}^{3(\delta-k)} \bigr]$
the only non-zero term is obtained for $l=\dim W_{S_1/D}^{3k}=2k$.
Therefore, we finally obtain
\begin{align*}
  c_{2\delta}(\mathcal{L}^{[3\delta]})
  \bigl[\mathcal{W}^{[3\delta]}_{\infty}\bigr]
  &= \sum_{k=0}^{\delta}
    c_{2k}(L_1^{[3k]})
    \bigl[W_{S_1/D}^{3k}\bigr]
    c_{2(\delta-k)}(L_2^{[3(\delta-k)]})
    \bigl[W_{S_2/D}^{3(\delta-k)}\bigr] \\
 & =\sum_{k=0}^{\delta}d_{k}\left(S_1/D,L_1\right)d_{\delta-k}\left(S_2/D,L_2\right),
\end{align*}
which ends the proof of Formula \eqref{eq:Tz-degen-formula-0}.
Formula \eqref{eq:Tz-degen-formula} follows at once.
\end{proof}


With Proposition \ref{proposition T3.9} at hand,
the proof of Theorem \ref{theorem T3.2} consists in using 
degenerations to the normal cone
(and Proposition \ref{proposition T3.9} itself)
in order to replace all
relative generating functions by absolute ones in
the degeneration formula
\eqref{eq:Tz-degen-formula}.
We will thus use several times the following lemma.

\begin{lemma}
\label{l:Tz-degen-normcone}
Let $S$ be a smooth surface, and $C \subset S$ be a smooth curve with
normal bundle $N_{C/S}$. 
Let $E\cong \P(\mathcal{O}_C\oplus N_{C/S})$, and $\eta: E \to C$ be
the $\P^1$-bundle map.
For all line bundles $L$ on $S$, we have
\begin{equation}
\label{eq T3.2_1}
\phi(S,L)=\phi(S/C,L)\cdot\phi(E/C,\eta^*(L|_{C})).
\end{equation}
\end{lemma}

\begin{proof}
Let us consider the degeneration of $S$ to $S\cup_C E$ constructed in
Example \ref{example blowup}, endowed with the line bundle $\cL$
obtained by pulling $L$ back (this is the case $k=0$ in 
Example \ref{example blowup}). On the degenerate fibre
$S\cup_C E$, one has
$\restr {\cL} S = L$
and $\restr {\cL} E = \eta^* \restr L C$.
Therefore, the degeneration formula \eqref{eq:Tz-degen-formula}
applied to this situation gives the required Formula \eqref{eq T3.2_1}.
\end{proof}


% \begin{proof}[Proof of Theorem \ref{theorem T3.2}]
\paragraph{}
{\itshape Proof of Theorem \ref{theorem T3.2}}.
We have
\begin{equation}
\label{eq:Tz-fin-0}
  \phi(S_0,L_0)=\phi(S_1/D,L_1)\cdot\phi(S_2/D,L_2).
\end{equation}
by Proposition \ref{proposition T3.9}.

By Lemma \ref{l:Tz-degen-normcone}, we have 
\begin{equation}
\label{eq T3.2_2}
\phi(S_i,L_i)=\phi(S_i/D,L_i)\cdot
\phi(E_i/D_i^-,\eta_i^*\restr {L_i} D)
\end{equation}
for $i=1,2$, where
$E_i:=\P(\mathcal{O}_D\oplus N_{D/S_i})$,
$\eta_i :E_i \to D$ is the $\P^1$-bundle map,
and $D_i^-:=\P(N_{X_i/D})$ and $D_i^+:=\P(\mathcal{O}_{D})$
are the two distinguished sections of $\eta_i$.
Now, the assumed extended double point relation tells us that
$S_3 \simeq E_i$, and $L_3\simeq \eta_i^*\restr \cL D$
for $i=1,2$, in the
notation introduced after Theorem \ref{theorem T3.2}.
Since $\restr \cL {S_i} = L_i$, we have
$L_3\simeq\eta_i^* \restr {L_i}{D}$, so that 
\eqref{eq T3.2_2} may be rewritten as
\begin{equation}
\label{eq T3.2_2bis}
\phi(S_i,L_i)=\phi(S_i/D,L_i)\cdot\phi(E_i/D_i^-,L_3).
\end{equation}

Finally, we apply Lemma \ref{l:Tz-degen-normcone} to the curve $D_1^-$
in the surface $E_1$; in this case, the degeneration to the normal
cone considered in the proof of the lemma is a degeneration of $E_1$
to $E_1\cup_D E_1$, where the curve $D$ is embedded as
$D_1^{-}$ in the first $E_1$, and as $D_1^{+}$ in the second $E_1$.
We obtain the identity
\begin{equation}
\label{eq T3.2_3}
\phi(E_1,L_3)=\phi(E_1/D_1^-,L_3)\cdot\phi(E_1/D_1^+,L_3).
\end{equation}
Since $E_1\simeq S_3$ on the one hand,
and on the other hand the isomorphism $(E_1,\eta_1^* \restr {L_1}{D})) \simeq
(E_2,\eta_2^* \restr {L_2} D)$ maps $D_1^{+}$ to $D_2^{-}$
(see Remark \ref{rk:S_1S_2}),
\eqref{eq T3.2_3} may be rewritten as
\begin{equation}
\label{eq T3.2_3bis}
\phi(S_3,L_3)=\phi(E_1/D_1^-,L_3)\cdot\phi(E_2/D_2^-,L_3).
\end{equation}

In conclusion, by
\eqref{eq:Tz-fin-0},
\eqref{eq T3.2_2bis},
and \eqref{eq T3.2_3bis}, we have
\[
  \phi(S_0,L_0)
  =
  \frac {\phi(S_1,L_1)} {\phi(E_1/D_1^-,\eta_1^*\restr {L_1} D)}
  \cdot
  \frac {\phi(S_2,L_2)} {\phi(E_2/D_2^-,\eta_2^*\restr {L_2} D)}
  =
  \frac {\phi(S_1,L_1) \cdot \phi(S_2,L_2)}
  {\phi(S_3,L_3)},
\]
as we wanted.
\qed
%\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Conclusion}\label{sub proofs}

This final section is dedicated to the proofs of
Theorems \ref{theorem G} and \ref{theorem T}.
The substantial work has already been done, and it remains only to
assemble the various pieces.

We first prove the analogue of Theorem \ref{theorem G} for the
generating function $\phi(S,L)=\sum d_{\delta}(S,L)x^{\delta}$, and
describe explicitly the universal power series involved.
Theorem \ref{theorem G} itself will follow rather directly, thanks to
Theorem \ref{theorem G5.2}.

\begin{proposition}\label{proposition T4.1}
For all pairs $(S,L)$, one has
\begin{equation*}
\phi(S,L)=A_1^{L^2}A_2^{LK_S}A_3^{K_S^2}A_4^{c_2(S)},
\end{equation*}
with
\begin{align*}
& A_1=\phi(\P^2, \mathcal{O}_{\P^2})^{-1}\phi(\P^2, \mathcal{O}_{\P^2}(1))\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1})^{\frac{3}{2}}\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1}(1,0))^{-\frac{3}{2}}, \\
& A_2=\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1})^{\frac{1}{2}}\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1}(1,0))^{-\frac{1}{2}}, \\
& A_3=\phi(\P^2, \mathcal{O}_{\P^2})^{-\frac{1}{3}}\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1})^{-\frac{1}{4}}, \\
& A_4=\phi(\P^2, \mathcal{O}_{\P^2})^{-\frac{2}{3}}\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1})^{\frac{3}{4}}.
\end{align*}
\end{proposition}

\begin{proof}
Given a class $[S,L]\in \omega_{2,1}$, Theorem \ref{theorem T2.3}
tells us that
$$
[S,L]=a_1[\P^2,\mathcal{O}_{\P^2}]+ a_2[\P^2,\mathcal{O}_{\P^2}(1)]+ a_3[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}]+a_4[\P^1\times\P^1,\mathcal{O}_{\P^1\times\P^1}(1,0)],
$$
with ${a_1=-L^2+\frac{K_S^2-2c_2(S)}{3}}$, ${a_2=L^2}$, ${a_3=\frac{3L^2+LK_s}{2}-\frac{K_S^2-3c_2(S)}{4}}$ and ${a_4=-\frac{3L^2+LK_S}{2}}$.
Then, Theorem \ref{theorem T3.2} yields 
$$
\phi(S,L)=\phi(\P^2,\mathcal{O}_{\P^2})^{a_1}\phi(\P^2, \mathcal{O}_{\P^2}(1))^{a_2}\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1})^{a_3}\phi(\P^1\times \P^1, \mathcal{O}_{\P^1\times \P^1}(1,0))^{a_4},
$$  
from which the assertion follows by replacing
$a_1,\dots,a_4$ with their expressions in terms of
$L^2$, $LK_S$, $K_S^2$, and $c_2(S)$.
\end{proof}


\begin{remark}
According to Remark \ref{remark basis}, we may easily determine an alternative basis of $\omega_{2,1}\otimes_{\Z}{\Q}$, and the corresponding coefficients of an arbitrary class $[S,L]\in \omega_{2,1}$ may be otained as in the proof of Theorem \ref{theorem T2.3}.
Consequently, the universal power series $A_1,A_2,A_3,A_4\in \Q[[x]]$ could be described in terms of any such basis.
\end{remark}

\begin{remark}\label{remark_5d-1}
Tzeng proved the G\"ottsche conjecture
% under the assumption that $L$ is $(5\delta-1)$-very ample line bundle
as follows (see \cite[Theorem 1.1]{T}).
She observed that by expanding the series $A_1,A_2,A_3,A_4$ in
Proposition \ref{proposition T4.1}, the coefficient $d_{\delta}(S,L)$
of $x^{\delta}$ in the generating function $\phi(S,L)$
is a universal polynomial $T_{\delta}$ of degree $\delta$ in the
variables $L^2,LK_S,K_S^2,c_2(S)$ (\cf \cite[Corollary 4.2]{T}),
\ie the analogue of the G\"ottsche conjecture holds for
the numbers $d_{\delta}(S,L)$,
without any positivity assumption on $L$.
Then, the conjecture for the numbers $a_{\delta}(S,L)$ follows by
Theorem \ref{theorem G5.2},
under a suitable positivity asumption
(Tzeng needed $(5\delta-1)$-very ampleness, but we now know that
$(3\delta-1)$-very ampleness suffices,
thanks to \cite{KST-12}, see Theorem \ref{theorem KST2.1}).
\end{remark}

\paragraph{\normalfont \itshape Proof of Theorem \ref{theorem G}}
% \begin{proof}[Proof of Theorem \ref{theorem G}]
Consider the generating function $T(S,L)$
% =\sum
% T_{\delta}(L^2,LK_S,K_S^2,c_2(S))x^{\delta}$
of the universal
polynomials $T_{\delta}(L^2,LK_S,K_S^2,c_2(S))$;
the existence of the latter is guaranteed by Theorem \ref{theorem KST}.
If $L$ is $(3\delta-1)$-very ample,
then Theorems \ref{theorem KST} and \ref{theorem G5.2} ensure that $T_{\delta}(L^2,LK_S,K_S^2,c_2(S))=a_{\delta}(S,L)=d_{\delta}(S,L)$.
Thus the generating functions $T(S,L)$ and $\phi(S,L)$ coincide, and we deduce from Proposition \ref{proposition T4.1} that $T(S,L)=A_1^{L^2}A_2^{LK_S}A_3^{K_S^2}A_4^{c_2(S)}$.
% \end{proof}
\qed


\bigskip\noindent
Finally, let us prove the G\"ottsche--Yau--Zaslow formula.

\paragraph{\normalfont \itshape Proof of Theorem \ref{theorem T}}
% \begin{proof}[Proof of Theorem \ref{theorem T}]
Let us consider the generating function
\begin{equation*}
\gamma(S,L)(q):=\sum_{\delta\geqslant 0}T_{\delta}(L^2,LK_S,K_S^2,c_2(S))\left(DG_2(\tau)\right)^{\delta}
\end{equation*}
appearing in the right-hand side of G\"ottsche--Yau--Zaslow formula.
Given two integers $g\geqslant\delta\geqslant 0$, let $(S,L)$ consist
of a very general $K3$ surface $S$ endowed with a primitive line
bundle $L$
such that $L^2=2(g+\delta-1)$, and let $M_g(\delta)$ denote the
number of curves in $|L|$ having geometric genus $g$ and passing
through $g$ general points of $S$ (or, equivalently, contained in a
general linear subsystem of $V\subset |L|$ of codimension $g$
and dimension $\delta$).  
Bryan and Leung \cite{BL-12})
(see \cite[Theorem \tref{T:BL}]{10.th-panoramico})
% \cite[Theorem 1.1]{BL-12})
proved that the generating function of the numbers $M_g(\delta)$
satisfies the formula 
\begin{equation*}
\sum_{\delta\geqslant 0}M_{g}(\delta)q^{g+\delta-1}=\frac{DG_2(\tau)^g}{\Delta(\tau)}
\end{equation*}
which, according to \cite[Remark 2.6]{G}, can be reformulated as
\begin{equation}\label{eq BL}
\gamma(S,L)(q)=\frac{\left(DG_2(\tau)/q\right)^{\chi(L)}}{\Delta(\tau)D^2G_2(\tau)/q^2}.
\end{equation}
On the other hand, we recall that the 4-tuples $(L^2,LK_S,K_S^2,c_2(S))$ and $(K_S^2,LK_S,\chi(L),\chi(\mathcal{O}_S))$ determine each other through linear relations (\cf Remark \ref{remark 4tuples}).
Since $\gamma(S,L)(q)$ coincides with the generating function $\phi(S,L)$ computed at $x=DG_2(\tau)$, we deduce from Proposition \ref{proposition T4.1} that there exist four universal power series $B_1(q),\dots,B_4(q)\in \Q[[q]]$ such that
\begin{equation}\label{eq B_i}
\gamma(S,L)(q)=B_1(q)^{K_S^2}B_2(q)^{LK_S}B_3(q)^{\chi(L)}B_4(q)^{\chi(\mathcal{O}_S)}.
\end{equation}
When $S$ is a $K3$ surface, equation \eqref{eq B_i} becomes $\gamma(S,L)(q)=B_3(q)^{\chi(L)}B_4(q)^{2}$. 
Moreover, as we consider different pairs $(S,L)$ such that $L^2=2(g+\delta-1)$, the latter equality must be satisfied for any positive integer $\chi(L)=g+\delta+1$.
Comparing $\gamma(S,L)(q)=B_3(q)^{\chi(L)}B_4(q)^{2}$ and \eqref{eq
  BL}, we then conclude that $B_3(q)=DG_2(\tau)/q$ and
$B_4(q)=\left(\Delta(\tau)D^2G_2(\tau)/q^2\right)^{-1/2}$.  Therefore
\eqref{eq B_i} leads to the G\"ottsche--Yau--Zaslow formula  
\begin{equation*}
\gamma(S,L)(q)=B_1(q)^{K_S^2}B_2(q)^{LK_S}\frac{\left(DG_2(\tau)/q\right)^{\chi(L)}}{\left(\Delta(\tau)D^2G_2(\tau)/q^2\right)^{\chi(\mathcal{O}_S)/2}}.
\end{equation*}
%\end{proof}
\qed


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{references}


% \begin{thebibliography}[Chapters in this Volume]{XIII}
\begin{thebibliography}[{Chapters in \thisVolume}]{XIII}


\bibitem[I]{01.ciro}
  C.~Ciliberto and Th.~Dedieu,
  \emph{Limits of nodal curves: generalities and examples}.

\bibitem[II]{02.edoardo}
Th.~Dedieu, E.~Sernesi, 
\emph{Deformations of curves on surfaces}.

\bibitem[VI]{04.concettina}
  Th.~Dedieu, C.~Galati,
  \emph{Degenerations and deformations of generalized Severi varieties}.

\bibitem[XI]{10.th-panoramico}
Th.~Dedieu,
\emph{Enumerative geometry of $K3$ surfaces}.

\bibitem[XII]{13.th-classic}
Th.~Dedieu,
\emph{Some classical formul{\ae} for curves and surfaces}.

\bibitem[XIII]{14.th-vainsencher}
Th.~Dedieu,
\emph{Node polynomials for curves on surfaces}.

\end{thebibliography}


\begin{thebibliography}[External References]{99}

\bibitem{block-goettsche-A-12}
F.~Block {\normalfont \smfandname} L.~G\"ottsche, \emph{Refined curve counting
  with tropical geometry}, Compos. Math. \textbf{152} (2016), no.~1, 115--151.

\bibitem{BL-12} J. Bryan, N. C. Leung, The enumerative geometry of K3 surfaces and modular forms, \emph{J. Amer. Math. Soc.} \textbf{13} (2000), 371--410.

\bibitem{CH-12} L. Caporaso, J. Harris, Counting plane curves of any genus, \emph{Invent. Math.} \textbf{131}(2) (1998), 345--392.

\bibitem{DH} S. Diaz, J. Harris, Ideals associated to deformations of
  singular plane curves, \emph{Trans. Amer. Math. Soc.} \textbf{309}
  (1988), 433--468.

\bibitem{DS-12}
Th.~Dedieu, E.~Sernesi, 
{Equigeneric and equisingular families of curves on surfaces},
\emph{Publ. Mat.} \textbf{61} (2017), no.~1, 175--212.

\bibitem{EGL} G. Ellingsrud, L. G\"ottsche, M. Lehn, On the cobordism class of the Hilbert scheme of a surface, \emph{J. Algebraic Geom.} \textbf{10} (2001), 81--100.

\bibitem{F} W. Fulton, \emph{Intersection theory}, Second edition, Ergeb. Math. Grenzgeb. (3) \textbf{2}, Springer-Verlag, Berlin (1998).

\bibitem{G} L. G\"ottsche, A conjectural generating function for numbers of curves on surfaces, \emph{Comm. Math. Phys.} \textbf{196} (1998), 523--533.

\bibitem{goettsche-shende-12}
L.~G\"ottsche {\normalfont \smfandname} V.~Shende, \emph{Refined curve counting
  on complex surfaces}, Geom. Topol. \textbf{18} (2014), no.~4, 2245--2307.

\bibitem{goettsche-shende2-12}
  \bysame ,
  \emph{The $\chi_{-y}$-genera of relative Hilbert schemes for linear
    systems on Abelian and $K3$ surfaces},
  Algebr. Geom. {\bf 2} (2015), no.~4, 405--421.

\bibitem{GLS-12} G.-M. Greuel, C. Lossen, E. Shustin, \emph{Introduction to singularities and deformations}, Springer Monographs in Mathematics, Springer, Berlin (2007).
%
\bibitem{Hart} R. Hartshorne, \emph{Algebraic geometry}, Graduate Texts in Mathematics {\bf 52}, Springer-Verlag, New York-Heidelberg (1977).

\bibitem{GH} P. A. Griffiths and J. Harris, \emph{Principles of Algebraic Geometry}, Pure and Applied Mathematics, Wiley Interscience, New York (1978).

\bibitem{KZ} M. Kaneko, D. Zagier, A generalized Jacobi theta function and quasimodular forms, in: \emph{The moduli space of curves (Texel Island, 1994)}, 165--172, Progr. Math. \textbf{129}, Birkhäuser Boston, Boston, MA (1995).

\bibitem{K-12} S. Kleiman, The transversality of a general translate, \emph{Compositio Math.} \textbf{38} (1974), 287--297.

\bibitem{KP1-12} S. Kleiman, R. Piene, Enumerating singular curves on surfaces, in: \emph{Algebraic geometry: Hirzebruch 70 (Warsaw, 1998)}, 209--238, Contemp. Math. \textbf{241}, Amer. Math. Soc., Providence, RI (1999).

\bibitem{KP2-12}
  \bysame , Node polynomials for families: methods and applications, \emph{Math. Nachr.} \textbf{271} (2004), 69--90.

\bibitem{KST-12} M. Kool, V. Shende, R. P. Thomas, A short proof of the G\"ottsche conjecture, \emph{Geom. Topol.} \textbf{15} (2011), 397--406.

\bibitem{laarakker}
T.~Laarakker, \emph{The {Kleiman}-{Piene} conjecture and node polynomials for
  plane curves in {{\(\mathbb{P}^3\)}}}, Sel. Math., New Ser. \textbf{24}
  (2018), no.~5, 4917--4959.

\bibitem{levine-morel}
M.~Levine {\normalfont \smfandname} F.~Morel, \emph{Algebraic cobordism},
  Springer Monographs in Mathematics, Springer, Berlin, 2007.

\bibitem{LevP} M. Levine, R. Pandharipande, Algebraic cobordism revisited, \emph{Invent. Math.} \textbf{176} (2009), 63--130.

\bibitem{LeeP} Y.-P. Lee, R. Pandharipande, Algebraic cobordism of bundles on varieties, \emph{J. Eur. Math. Soc. (JEMS)} \textbf{14} (2012), 1081--1101.

\bibitem{li-jdg}
J.~Li, \emph{A degeneration formula of {GW}-invariants}, J. Differential Geom.
  \textbf{60} (2002), no.~2, 199--293.

\bibitem{li-handbook}
\bysame , \emph{Good degenerations of moduli spaces}, in \emph{Handbook of
  moduli. {V}ol. {II}}, Adv. Lect. Math. (ALM), vol.~25, Int. Press,
  Somerville, MA, 2013, 299--351.

\bibitem{LW} J. Li, B. Wu, Good degeneration of Quot-schemes and coherent systems, \emph{Comm. Anal. Geom.} \textbf{23} (2015), 841--921.

\bibitem{LT} J. Li, Y.-J. Tzeng, Universal polynomials for singular curves on surfaces, \emph{Compos. Math.} \textbf{150} (2014), 1169--1182.

\bibitem{Liu1} A.-K. Liu, Family blowup formula, admissible graphs and the enumeration of singular curves, I, \emph{J. Differential Geom.} \textbf{56} (2000), 381--579.

\bibitem{Liu2}
  \bysame , The algebraic proof of the universality theorem, preprint, arXiv:math.AG/0402045 (2004).

\bibitem{Macdonald} I.~G.~Macdonald, 
Symmetric products of an algebraic curve,
\emph{Topology} {\bf 1} (1962), 319--343.

\bibitem{PT} R. Pandharipande, R. P. Thomas, Stable pairs and BPS invariants, \emph{J. Amer. Math. Soc.} \textbf{23} (2010), 267--297.

\bibitem{rennemo-12}
J.~V. Rennemo, \emph{Universal polynomials for tautological integrals on
  {H}ilbert schemes}, Geom. Topol. \textbf{21} (2017), no.~1, 253--314.

\bibitem{S} V. Shende, Hilbert schemes of points on a locally planar curve and the Severi strata of its versal deformation, \emph{Compos. Math.} \textbf{148} (2012), 531--547.
\bibitem{T} Y.-J. Tzeng, A proof of the G\"ottsche--Yau--Zaslow formula, J. Differential Geom. \textbf{90} (2012), 439--472.
\bibitem{Vei} I. Vainsencher, Enumeration of $n$-fold tangent hyperplanes to a surface, \emph{J. Algebraic Geom.} \textbf{4} (1995), 503--526.
\bibitem{Vak} R. Vakil, Counting curves on rational surfaces, \emph{Manuscripta Math.} \textbf{102} (2000), 53--84.
\bibitem{V2} C. Voisin, \emph{Hodge theory and complex algebraic geometry II}, Cambridge Studies in Advanced Mathematics \textbf{77}, Cambridge University Press, Cambridge (2007).

\bibitem{YZ-12} S. T. Yau, E. Zaslow, BPS states, string duality, and nodal curves on K3, \emph{Nuclear Phys. B} \textbf{471} (1996), 503--512.

\end{thebibliography}

\end{references}

% \bibliographystyle{mysmf-alpha}
% \bibliography{goettsche_add}

\vfill

\stopcontents[12.fra-goettsche]

% \end{document}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main.tex"
%%% coding: utf-8
%%% End: 
 	

